An Approximation Algorithm for the Art Gallery Problem

Given a simple polygon $\mathcal{P}$ on $n$ vertices, two points $x,y$ in $\mathcal{P}$ are said to be visible to each other if the line segment between $x$ and $y$ is contained in $\mathcal{P}$. The Point Guard Art Gallery problem asks for a minimum set $S$ such that every point in $\mathcal{P}$ is visible from a point in $S$. The set $S$ is referred to as guards. Assuming integer coordinates and a specific general position assumption, we present the first $O(\log \text{OPT})$-approximation algorithm for the point guard problem for simple polygons. This algorithm combines ideas of a paper of Efrat and Har-Peled [Inf. Process. Lett. 2006] and Deshpande et. al. [WADS 2007]. We also point out a mistake in the latter.

==> Approx.tex <==


\begin{definition}[polygon representation, width, grid]
   Given a polygon $\mathcal P$, we will always assume that all its 
  vertices are given by \emph{positive} integers in binary.
  We denote by $L$ \emph{twice} the \emph{largest distance} between any two vertices of $\mathcal P$ rounded up. The value $L$ is larger than the diameter of $\mathcal P$.  Note that $L$ is at most four times as large as the largest integer of any vertex of the polygon. Thus $\log L$ is linear in the input size.
  We set the width to $w = L^{-10}$ and define the grid $\Gamma$ as 
  $(w\cdot \mathbb{Z}^2) \cap \mathcal{P}$. Note that all vertices of $\mathcal P$ have integer coordinates and thus are included in $\Gamma$. We denote by $OPT$ an optimal solution of the \pgag problem and by $k$ its size.
  We denote by $OPT_\textup{grid}$ an optimal solution of the \textsc{Grid Guard Art Gallery Problem}, this is, guards are restricted to lie on the grid $\Gamma$, and by $k_\textup{grid}$ its size.
\end{definition}


The idea is to show that the algorithm of Efrat and Har-Peled gives an approximation algorithm under the integer vertex representation assumption and the grid $\Gamma$ as described above.

\begin{theorem}[Efrat,Har-Peled~\cite{DBLP:journals/ipl/EfratH06}]
  Given a simple polygon $\mathcal P$ with $n$ vertices, one can spread a grid $\Gamma$ inside $\mathcal P$ , and compute an $O(\log k_\textup{grid})$-approximation to the smallest subset of $\Gamma$ that sees $\mathcal P$. The expected running time of the algorithm is $O(n \, k_\textup{grid}^2  \log  k_{grid} \, \log( n k_\textup{grid}) $ $  \, \log^2 \Delta)$,
  where $\Delta$ is the ratio between the diameter of the polygon and the grid size.
\end{theorem}
Note that the grid size equals $w = L^{-10}$, thus $\Delta \leq L^{11}$ and consequently $\log \Delta \leq 11 \log L$, which is polynomial in the size of the input. 

It remains to show the following lemma.
\begin{lemma}\label{lem:GridReplacement}
  $k_\textup{grid} \leq 6k.$
\end{lemma}

The way we use the integer coordinate assumption is to infer distance lower bounds between various objects of interest. The proofs are technical and not very enlightening, fortunately they are short.

\begin{lemma}[Distances]\label{lem:distances}
  Let $\mathcal P$ be a polygon with integer coordinates and $L$ be some upper bound one the largest integer representing vertices of $\mathcal P$.
  Let $v$ and $w$ be vertices of $\mathcal P$, $\ell$ and $\ell'$ supporting lines of two vertices, and $p$ and $q$ intersections of supporting lines.
  \begin{enumerate}
   \item \label{itm:VertexVertex} $\dist(v,w)>0 \Rightarrow \dist(v,w)\geq 1$.
   \item \label{itm:VertexLine}$\dist(v,\ell) >0 \Rightarrow \dist(v,\ell) \geq 1/L$.
   \item \label{itm:IntersectionLine}$\dist(p,\ell) >0 \Rightarrow \dist(p,\ell) \geq 1/L^5$.
   \item \label{itm:IntersectionIntersection}$\dist(p,q) >0 \Rightarrow \dist(p,q) \geq 1/L^4$.
   \item \label{itm:parralelLines} Let $\ell\neq \ell'$ be parallel. Then $\dist(\ell,\ell') \geq 1/L$.
   \item \label{itm:NonParralelLines} Let $\ell$ and $\ell'$ be non-parallel and $a$ and $a'$ points on $\ell$ and $\ell'$ respectively, with $\dist(a,a') \leq d$. Then for the intersection $p$ of $\ell$ and $\ell'$ holds $a,a'\in \disk(p,dL^2)$.
  \end{enumerate}
\end{lemma}

% See the appendix for a proof of this lemma.

% \appendixproof{Lemma~\ref{lem:distances}}{
\begin{proof}
  Case~\ref{itm:VertexVertex} seems trivial, but follows the same general principal as the other bounds.
  All these distances, are realized by geometric objects, and these geometric objects are represented with the help of the input integers.
  In order to compute theses distances some elementary calculations are performed and solutions can be expressed as fractions of the input integers. Using the lower bound one and the upper bound $L$ or $L/2$ on these integers or derived expressions give the desired results.
  
  Consider Case~\ref{itm:VertexLine}. Let $\ell$ be the supporting line of $w_1$ and $w_2$. 
  The distance $d$ between $v$ and $\ell$ can be expressed as $\tfrac{|(v-w_1)\cdot (w_2-w_1)^{\bot}|}{\|w_2-w_1\|}$, where $\binom{x_1}{x_2}^{\bot} = \binom{x_2}{-x_1}$ represents the orthogonal vector to $x$ and $\cdot$ indicates the dot product. 
  As $v$ is not on $\ell$ the nominator is lower bounded by one. The denominator is upper bounded by the diameter $L$.
  
  Consider Case~\ref{itm:IntersectionLine}. Let $p$ be the intersection of $\ell_1 = \ell(v_1,v_2)$ and $\ell_2 = \ell(u_1,u_2)$. Then $p$ is the unique solution to the linear equations 
  $(u_2-u_1) \cdot (p-u_1)=0 $ and 
  $(v_2-v_1) \cdot (p-v_1)=0 $.
  So let us write this as an abstract linear equation $A\cdot x = b$.
  By Cramer's rule holds $x_i = \tfrac{det(A_i)}{det(A)}$, for $i = 1,2$.
  Here $det()$ is the determinant and $A_i$ is the matrix with the $i$-th column replaced by $b$. It is easy to see that $det(A)$ is bounded by $L^2$. 
  Let $\ell=\ell(w_1,w_2)$ be a different line.
  Observe that the points $w_1$, $w_2$ and $p$ lie on a grid $\Gamma^*$ of width $1/det(A)$. 
  After scaling everything with $det(A)$ the diameter $L^*$ of this grid becomes $det(A) L \leq L^3$. Thus by Case~\ref{itm:VertexLine} the distance between the line $\ell$ and the grid point $p$ is lower bounded by $(1/L^*) \geq 1/L^3$. Scaling everything back by $1/det(A)\geq L^{-2}$ yields the claimed bound.
  
  Consider case~\ref{itm:IntersectionIntersection}. 
  Let $p$ be the intersection of $\ell_1 = \ell(v_1,v_2)$ and $\ell_2 = \ell(u_1,u_2)$.
  And likewise let $q$ be the intersection of $\ell_3 = \ell(w_1,w_2)$ and $\ell_2 = \ell(t_1,t_2)$. Then $p$ is the unique solution to the linear equations 
  $(u_2-u_1) \cdot (p-u_1)=0 $ and 
  $(v_2-v_1) \cdot (p-v_1)=0 $.
  So let us write this as an abstract linear equation $A\cdot x = b$.
  By Cramer's rule holds $x_i = \tfrac{det(A_i)}{det(A)}$, for $i = 1,2$.
%   Here $det()$ is the determinant and $A_i$ is the matrix with the $i$-th column replaced by $b$. 
  Thus the coefficients of $p-q$ can be represented by $\tfrac{a}{det(A)\cdot det(A')}$ for some value $a\neq 0$ and some matrices $A$ and $A'$. Note that $det(A)$ and $det(A')$ are bounded by   $L^2$ from above.
  
  Case~\ref{itm:parralelLines} follows from Case~\ref{itm:VertexLine} as follows. Let $\ell'=\ell(w_1,w_2)$. Then $\dist(\ell,\ell') = \dist(\ell,w_1)\geq 1/L$.
  
  
  \begin{figure}[htbp]
    \centering
    \includegraphics{NonParralelLines}
    \caption{}
    \label{fig:NonParralelLines}
  \end{figure}
  For case~\ref{itm:NonParralelLines}, see Figure~\ref{fig:NonParralelLines} and the notation therein. To be more explicit, we rotated the plane till $\ell$ is horizontal. Without loss of generality assume that $\dist(a,p)\geq \dist(a',p)$. It remains to show $a\in \disk(p,dL)$.
  The distance $d$ between $a$ and $a'$ is clearly longer than the vertical distance between $a$ and $\ell'$. We denote by $m$ the slope of $\ell'$ after the described rotation. We set $x = d/ |m|$.   Note that $m$ can be computed by $|m| = \tfrac{\|(v_2-v_1)\times (w_2-w_1)\|}{\| (v_2-v_1) \|\cdot \| (w_2-w_1) \|} \geq \frac{1}{L^2}$. This implies $x = d/|m|\leq d L^2$.
\end{proof}
% }
 
\begin{definition}[Local Visibility Containment Property]
  Given a point $x$ and two points $r_1,r_2$ in the plane, we define the cone of $x$ with respect to $r_1$ and $r_2$ as the unique cone with apex $x$ that is bounded by $r_1$ and $r_2$ and forms an angle smaller than $\pi$. 
  
  Given four points $g_1,g_2,g_3,g_4$ of a grid-cell $C$ of $\Gamma$ and a point $x\in C$, we denote by $\textup{grid}(x)$ the grid points of the cell containing $x$.
  We say $x$ is \emph{safe} with respect to a pair of opposite reflex vertices $r_1$ and $r_2$, if
  the cone of $x$ with respect to $r_1$ and $r_2$ is contained in the cones of  $g_1,g_2,g_3,g_4$.
  We say, the grid cell $C$ is safe, if it is safe with respect to every point $x\in C$ and every pair of reflex vertices.
  
  We say a grid cell $C$ with vertices $g_1,g_2,g_3,g_4$ has the \emph{local visibility containment property} if for all $x\in C:$ $V(x)\subseteq V(g_1)\cup V(g_2)\cup V(g_3)\cup V(g_4)$.
\end{definition}


\begin{definition}[opposite reflex vertices,thin bad regions]
  Given a polygon $\mathcal P$ and two reflex vertices $r_1$ and $r_2$, consider the supporting line $\ell = \ell(r_1,r_2)$ restricted to $\mathcal P$ and assume it connects $r_1$ and $r_2$. 
  The supporting line defines two halfplanes $\ell^+$ and $\ell^-$. 
  We say $r_1$ is \emph{opposite} of $r_2$ if $(D(r_1,\varepsilon)\cap \partial \mathcal{P})\subset \ell^+$
  and $(D(r_2,\varepsilon)\cap \partial P)\subset \ell^-$ for some small enough $\varepsilon>0$.
%   See Figure~\ref{fig:BadRegionDef}, for an illustration.

%   Given two opposite reflex vertices $r_1$ and $r_2$, let $\ell = \ell(r_1,r_2)$ be their supporting line. We define $S$ to be the stripe around $\ell$ of width $8wL$ and the \emph{bad region} of $r_1$ and $r_2$ as $S\cap \mathcal{P}$ and denote it by $BR(r_1,r_2)$. 
%   We denote by $BR$ the union of all bad regions together.
% %   See Figure~\ref{fig:BadRegionDef}, for an illustration.

  Given two opposite reflex vertices $r_1$ and $r_2$, we define their \emph{$\alpha$-bad regions} as the union of the two open triangles as in Figure~\ref{fig:ThinBadRegions}. Where, we set the slope as $\alpha$.

\end{definition}


%  \appendixtext{Figure~\ref{fig:BadRegionDef}}{
\begin{figure}[htbp]
  \centering
  \includegraphics{ThinBadRegions}
  \caption{Illustration of opposite reflex vertices and bad regions.}
  \label{fig:ThinBadRegions}
\end{figure}
% }



% \begin{lemma}\label{lem:safe}
%   Every grid cell $C$ outside the bad region of two reflex vertices is safe with respect to these reflex vertices.
% \end{lemma}
% 
% \begin{proof}
%   We fix some point $x\in C$  and  reflex vertices $r_1$ and $r_2$. It suffices to show safeness of $x$ with respect to $r_1$ and $r_2$.
%   Without loss of generality, assume that the supporting line of the two reflex vertices is horizontal.
%   In case that some grid point of $C$ is contained in the cone of $x$, we are done. So without loss of generality, we  assume that the situation up to relabeling is as depicted in Figure~\ref{fig:Cones}.



% 
%   It is sufficient to show that the rays $R_1 =\ray(g_1,r_1)$ and $R_2= \ray(g_2,r_2)$ will not intersect,
%   this is they are either parallel or diverge from one another.
%   For this purpose, we distinguish two different cases. Either the angle between the segment $\seg(r_1, r_2)$ and the supporting line of $x$ and the midpoint of $s$ is larger or equal to $45$ degree or smaller than $45$ degree.
%   
%   
%   In the first case, we compare the \emph{horizontal} distance between the rays at the apex and at the reflex vertices. The horizontal distance $h$ at the apex is at most $2w$ and the distance at the reflex vertices is at least $1$, by the assumption that all coordinates of the vertices are given by integers.
%   
%   In the second case, we compare the \emph{vertical} distance between the rays at the apex and at the reflex vertices.
%   The horizontal distance at the apex is at most $2w$. For the vertical distance $d$ at the reflex vertices consider Figure~\ref{fig:Safe} and the notation therein.
%   \begin{figure}[hbtp]
%     \centering
%     \includegraphics{LatexApproximation/figures/Safe2}
%     \caption{}
%     \label{fig:Safe}
%   \end{figure}
%   As the two triangles in the figure are homothetic\footnote{They are uniformly scaled versions of one another.}, it follows $\frac{d}{c} = \frac{b}{a}$, which is equivalent to $d = bc/a \geq 4wL \cdot 1 / L = 4w$. This finishes the proof.
% \end{proof}

%  \begin{figure}[htbp]
%   \centering
%  \includegraphics{LatexApproximation/figures/Cones2}
%  \caption{}
%  \label{fig:Cones}
% \end{figure}


\begin{lemma}\label{lem:ThinRegionsSafe}
  Every grid-cell $C$ outside the $4w$-bad region of two reflex vertices is safe with respect to these reflex vertices.
\end{lemma}
\begin{proof}
  We fix some point $x\in C$  and  reflex vertices $r_1$ and $r_2$. It suffices to show safeness of $x$ with respect to $r_1$ and $r_2$.
  Without loss of generality, assume that the supporting line of the two reflex vertices is horizontal.
  \begin{figure}[hbtp]
    \centering
    \includegraphics{Cones2}
    \caption{}
    \label{fig:Cones}
  \end{figure}
  In case that some grid point of $C$ is contained in the cone of $x$, we are done. So without loss of generality, we  assume that the situation up to relabeling is as depicted in Figure~\ref{fig:Cones}.
  It is sufficient to show that the rays $R_1 =\ray(g_1,r_1)$ and $R_2= \ray(g_2,r_2)$ will not intersect,
  this is they are either parallel or diverge from one another.
  For this purpose, we distinguish two different cases. Either the angle between the segment $s(r_1, r_2)$ and the supporting line of $x$ and the reflex vertex further away from $x$ is larger or equal to $45$ degree or smaller than $45$ degree.
  
  In the first case, we compare the \emph{horizontal} distance between the rays at the apex and at the reflex vertices. The horizontal distance $h$ at the apex is at most $2w$ and the distance at the reflex vertices is at least $1$, by the assumption that all coordinates of the vertices are given by integers.
  
  
  \begin{figure}[hbtp]
  \centering
 \includegraphics{Safe3}
 \caption{}
 \label{fig:Safe3}
\end{figure}

  In the second case, we compare the \emph{vertical} distance $d$ between the rays at the apex and at the reflex vertices.
  The horizontal distance at the apex is at most $1.5\cdot w$. For the vertical distance $d$ at the reflex vertices consider Figure~\ref{fig:Safe3} and the notation therein. To be explicit, $a$ denotes the distance between the two reflex vertices and is lower bounded by one. The variable $b$ indicates the horizontal distance between $x$ and the closer reflex vertex. The vertical distance between $x$ and the supporting line of the reflex vertices is denoted by $c$.
  As $x$ is outside the bad region, we know $c\geq 4w b$. 
  We observe that the triangles $\Delta_1$ and $\Delta_2$ as in Figure~\ref{fig:Safe3} are homothetic and it follows $\frac{d}{a}=\frac{c}{b+a}\Leftrightarrow d = \frac{c a }{b+a} \geq \frac{4wb a }{b+a} \geq \frac{4w b \cdot 1 }{b+a} \geq \frac{4w b  }{b+b} \geq 2w$.
  
\end{proof}





\begin{lemma}\label{lem:localVisibilityContainment}
  A grid cell, that is safe with respect to every pair of reflex vertices has the local visibility containment property.
\end{lemma}
% See the appendix for a proof of this lemma.

% \appendixproof{Lemma~\ref{lem:localVisibilityContainment}}{
\begin{proof}
 Assume there is a point $x$ that is safe, but has not the local visibility containment property. This is, there is a point $a$ that is seen by $x$ but not by the surrounding grid points $g_1,g_2,g_3,g_4$.
 Then, there exist at least two reflex vertices $r_1$ and $r_2$ that block the visibility between the gris points and $x$. It is easy to see that this implies that $x$ is not safe with respect to these reflex vertices (see Figure~\ref{fig:NotSafe}).
\begin{figure}[hbtp]
  \centering
 \includegraphics{NotSafe}
 \caption{}
 \label{fig:NotSafe}
\end{figure}
\end{proof}
% }

\begin{lemma}
  Every grid cell outside the bad region has the local visibility containment property.
\end{lemma}
\begin{proof}
  Every grid cell outside the bad regions is safe and being safe implies the local visibility containment property.
\end{proof}



\begin{lemma}\label{lem:conesSuppDist}
  Given a cone $C$ of a supporting line $\ell$ and $q$ be some point on the ``other side'' of $\ell$. Then there exists some $\varepsilon>0$ such that $\disk(q,\varepsilon)$ and $C$ are disjoint.
  Consequently, if $p$ is on the intersection of $t$ supporting lines, then there exists some $\varepsilon>0$ such that $\disk(q,\varepsilon)$ is disjoint from all the cones.
\end{lemma}
\begin{proof}
 Look at Figure~\ref{fig:DeshpandeCounterExample}.
\end{proof}

\begin{example}[Counter Example Deshpande et. al~\cite{DeshpandeThesis, DeshpandeWADS2007}]
    It is easy to believe that the local visibility containment property also holds inside the bad region.
    However this is not true. Here, we will describe a counter example briefly.
    In particular, this example shows that the algorithm of Deshpande et. al is not correct as it is stated. However, we want to mention that their paper nevertheless had ideas that motivated the algorithm presented in this paper.
    
    \begin{figure}[htbp]
      \centering
      \includegraphics{DeshpandeCounterExample}
      \caption{}
      \label{fig:DeshpandeCounterExample}
    \end{figure}

    
    See Figure~\ref{fig:DeshpandeCounterExample}, for the following description. We have two opposite reflex vertices with supporting line $\ell$. The points $(a_i)_{i\in \mathbb{N}}$ are chosen closer and closer to $\ell$ on the right side of the polygon. It is easy to see that non of the $a_i$ can see $t$, as this would require to be actually on $\ell$. Further, it is easy to see that the visible interval next to $t$ gets smaller and smaller as well. In fact, we choose the $(a_i)_{i\in \mathbb{N}}$ in a way that their intervals will be all disjoint. 
    
    Consider now a grid $\Gamma$ with arbitrary, but fixed width. And any finite collection $C\subset \Gamma$ in the vicinity of the $(a_i)_{i\in \mathbb{N}}$. We will show that there is some $a_i$, which sees some interval close to $t$, that is not seen by any point in $C$. Recall that no point sees the entire interval around $t$, but the visibility of the $a_i$ come arbitrarily close to $t$. Thus there is some $a_i$ that sees something that is not visible by any of the surrounding grid points. \qed
\end{example}
  

\begin{definition}[Evil-Cones]
  Given two opposite reflex vertices $r_1$ and $r_2$ and a point $x$ in the bad region of them, we define the \emph{evil cone} of $x$ with respect to $r_1$ and $r_2$, as 
  the region visible from $x$ on the other side of the diagonal $r_1r_2$, see Figure~\ref{fig:EvilCone}.
  We define the \emph{width of a cone} as the maximum distance between the two bounding rays within the polygon.
\end{definition}
\begin{figure}[htbp]
  \centering
  \includegraphics{EvilCone}
  \caption{}
  \label{fig:EvilCone}
\end{figure}
  Note that a point has an evil cone for each bad regions it lies in.

\begin{lemma}[Thin Evil Cones]
  The width of any evil cone is bounded by $4wL^2$.
\end{lemma}
\begin{proof}
  Let $x$ be in a bad region as in Figure~\ref{fig:EvilCone}. 
  Let $\Delta$ be the triangle as indicated in Figure~\ref{fig:EvilCone},
  with end vertices $a,b$ and $r_1$. The segment $seg(a,r_1)$ forms a slope of $4w$, with the line of $support(r_1,r_2)$.
  Beyond the diagonal $seg(r_1,r_2)$, the evil cone is contained in $\Delta$. As the distance between $r_1$ and $a$ is at most $L$, the evil cone has a width of at most $4wL$.
\end{proof}


\begin{lemma}\label{lem:EvilConesVisibility}
  Given $k$ evil cones and $D=disk(a,wL^4)$, then there is a point $b$ in $D$ no covered by the evil cones.
\end{lemma}
\begin{proof}
  Given $k$ evil cones with width $w_1,\ldots,w_k$, the $i$-th cone covers at most an area of $2r w_i \leq 2wL^4 \cdot 4wL^2 = 8w^2 L^6$ inside $D$.
  The area of $D$ equals $\pi r^2  \geq w^2 L^8 \gg k\cdot 8w^2 L^6$.
\end{proof}


\begin{definition}[far grid points]
  Given a point $x\in P$, we define the \emph{far grid} points of $x$ as the four points $g_1,g_2,g_3,g_4 \in \Gamma$ around $x$ 
  forming a aquare with sidelength $wL^2$, see Figure~\ref{fig:FarGridAndThinBadRegions}~b)
\end{definition}


\begin{lemma}[Augmenting Visibility]\label{lem:AugmentingVisibility}
  Let $y$ be a guard and $b$ be a point visible from $y$ with distance at least $L^{-1}$ from any reflex vertx.
  Let $disk(b,wL^5)$ be a large ball around $b$. Then $disk(b,..)$ is visible from the far grid points of $y$.
  
  Let $y\in \mathcal{P}$ be a point with visibility cone of width $d$ at least $\overline{w} L^2$ , then the far grid points see a cone of width at least $d + . ? .\tfrac{\overline{w}}{L^2}$
\end{lemma}
\begin{proof}
 to be filled
\end{proof}


\begin{lemma}
  Let $x$ be a guard and $a$ a point in an evil-cone of $x$ then there is another guard $y$ that sees $a$.
\end{lemma}
\begin{proof}
  Consider a large enough ball $B$ around $a$. There is a point $b\in B$ seen by a different guard $y$ such that $b$ is not in an evil cone of $y$, see Lemma~\ref{lem:EvilConesVisibility}
  Then the far grid points of $y$ see $B(b,..)$, which contains $a$.
  This finishes the proof.
\end{proof}

\begin{figure}
  \centering
  \includegraphics{ConeDistance}
  \caption{}
  \label{fig:ConeDistance}
\end{figure}

See Figure~\ref{fig:ConeDistance} for the following definition.
\begin{definition}[To cone width and cone supporting line distance]
 Let $x$ be some guard and $\textrm{Cone}(x)$ be its cone with respect to opposite reflex vertices $r_1$ and $r_2$. Further, let $\ell_{\text{orth}}$ be some line orthogonal to $\ell = \ell (r_1,r_2)$. We assume $\ell$ to be horizontal for the following.
 We define from top to bottom the points $a$ and $b$ as the endpoints of the segments defined by $\textrm{Cone}(x)\cap \ell_{\text{orth}}$ and $c$ as the intersection of $\ell$ and $\ell_{\text{orth}}$.
 We define $d = \|a-b\|$  and $e = \|a - c\|$.
\end{definition}


\begin{lemma}[supporting line distance]\label{lem:DistSupLine}
   We show:
 \[ d\leq . . . \Rightarrow e \leq . . .\]
\end{lemma}
\begin{proof}
  To be filled
\end{proof}

\begin{figure}
  \centering
  \includegraphics{IntersectionsSeenByBigCones}
  \caption{}
  \label{fig:IntersectionsSeenByBigCones}
\end{figure}


\begin{lemma}
  Let $p\in \mathcal{P}$ and $\ell$ the supporting line $\ell = \ell(r_1,r_2)$ of some pair of reflex vertices with distance $\textrm{dist}(p,\ell) \geq L^{-5}$ and $y\in \mathcal{P}$ be a point that sees $p$ and the cone of $y$ that sees $p$ is bounded by $r_1$ and $r_2$. Then the width $d$ of the cone of $y$ is at least . . . $L^{-10}$.
\end{lemma}
\begin{proof}
 To be filled
\end{proof}


\begin{lemma}[no three bad regions intersect]\label{lem:NoBadIntersection}
  There exists no point $p$ in $\mathcal P$ that belongs to three different bad regions.
\end{lemma}
% \appendixproof{Proof to Lemma~\ref{lem:NoBadIntersection}}{
\begin{proof}
%   
  Let $\ell_1,\ell_2,\ell_3$ be supporting lines of opposite reflex vertices.
  We want to show that the intersection of their corresponding bad regions is empty.
  These three lines form a triangle $\Delta$ with vertices of pairwise distance at least $L^{-4}$ by Lemma~\ref{lem:distances}. And by the same Lemma each vertex has distance at least $L^{-5}$ by Lemma~\ref{lem:distances}. Using elementary geometry it is easy to show that there exists now point inside $\Delta$ that has distance less than $w\cdot L \leq L^{-5}$ from all lines.
  But the bad regions are at most $4wL \leq L^{-8}$ away from their defining lines.
%   
%   
%   
%   Define $q_{ij} = \ell_i\cap \ell_j$, for $i< j \in \{1,2,3\}$.
%   We know that $dist(q_{ij},q_{i',j'}) \geq 1/L^4$ and $dist(q_{ij},\ell_m) \geq 1/L^2$ by Lemma~\ref{lem:distances}, for $(i,j)\neq (i',j')$ and $m\neq i,j$.
%   
\end{proof}
% }

\begin{proof}[Proof of Lemma~\ref{lem:GridReplacement}.]
  Let $OPT$ be an optimal solution of size $k$. We construct a set of $6k$ guards $G\subset \Gamma$, which see the entire polygon.
  For each guard $x\in OPT$, we add the four grid points surrounding $x$ into $G$.
  Further, if $x$ is in one or two bad regions, add a reflex vertex for each bad region into $G$.  For each $x\in OPT$ the local containment property holds, except for the bad regions it is in. These parts are seen by the reflex vertices we added.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:GridReplacement} without general position assumption]
 
 For now, only a sketch:
 
 For every point $x$ of OPT pick four grid points around $x$ and four \emph{far-grid} points around $x$ to our set $G\subseteq \Gamma$. Obviously $|G|\leq 8 |OPT|$.
 We will show that $G$ sees the entire polygon.
 
 Let $x\in OPT$, then for every pair of reflex vertices for which $x$ is safe, the grid points surrounding $x$ see as much as $x$.
 
 Let $x$ be a point that is in some bad region with respect to $r_1$ and $r_2$ and $\ell = \ell(r_1,r_2)$. Then we cannot guarantee that the grid points around $x$ see the cone of $x$ behind $\seg(r_1,r_2)$. Let $a\in \textrm{Cone}(x)$. We will show that $a$ is seen by some other far grid points of some other point $y\in OPT$.
 
 As $x$ is in a bad region we know that the width of $\textrm{Cone}(x)$ is at most $wL^2$. Let $D = disk(a,4wL^2)$. Then $\textrm{Cone}(x)$ does not cover $D$. 
 Let $C_1,\ldots,C_t$ be the visibility cones covering $D$ with width $\beta_1,\ldots, \beta_t$ respectively.
 It is easy to argue that $t$ is greater or equal to $2$.
 
 We consider two cases. 
 Case $1$: there exists a cone $C_i$ with width $\beta_i \geq \overline{w}L^2 = wL^6$.
 Case $2$: for all cones $j= 1,\ldots,t$ hmm $\beta_j <\overline{w}L^2 = wL^6$. 
 
 In case $1$, the far grid points around $C_i$ see at least $...$ more. This covers the whole disk $D$ and in particular the point $a$.
 
 In case $2$, by Lemma~\ref{lem:fig:DistSupLine} all the supporting lines $\ell_1,\ldots, \ell_t$ intersect a disk $D=\disk(a,f(w,L))$.
 
 \till{The radius here should be somewhat larger than before, but still depend on $w$}
 
 By Lemma~\ref{lem:distances}, all these lines have to intersect in a point $p \in \disk(a,f(w,L))$.
 
 \till{The radius here should be even larger than before, but still depend on $w$}
 
 There is some $\varepsilon>0$ such that none of the cones $C_1,\ldots,C_t$ covers the disk $D'= \disk(p,\varepsilon)$, by Lemma~\ref{lem:conesSuppDist}. 
 Thus there exists at least one different cone $\overline{C}= C(y)$ that covers $D'$ at least partially. Thus the corresponding supporting line $\overline{\ell}$ has distance at least $L^{-5}$ from $p$ as it does not intersect with $p$, see Lemma~\ref{lem:distances}. This implies that the cone has width at least $f(L)$.
 Thus the cone must be good with respect to its reflex vertices and the far grid points.
 Therefore, by Lemma~\ref{lem:AugmentingVisibility}, the cone $C_{\textrm{far}(y)}$ of the far grid points of $y$ is augmented at least by $F(w,L)$ and thus also covers $a$.
\end{proof}




% \begin{lemma}
%   Dropping the general position assumptions, it still holds:
%   $k_{\textup{grid}} \leq k^2 + 3k$
% \end{lemma}
% \begin{proof}
%   Let $v$ be a point in $t$ different bad regions defined by $t$ pairs of reflex vertices.
% %   $(r_a^1,r_b^1),\ldots,(r_a^t,r_b^t)$. 
%   The diagonals defined by 
%   these reflex vertices decompose the polygon into $t+1$ polygons $\mathcal{P}_1,\ldots, \mathcal{P}_{t+1}$ and no finite set of vertices of $\mathcal{P}_i$ can see a polygon $\mathcal{P}_j$ entirely, with $i\neq j$.
%   Thus the existence of such a point implies $k \geq t+1$.
%   
%   Let $OPT$ be an optimal solution, we select for each $x\in OPT$ the $4$ surrounding grid points plus one reflex vertex for each bad region that $x$ belongs to. Let $t$ be the maximal number of bad regions a vertex of $OPT$ belongs to then we selected at most $t\cdot k + 4k\leq (k-1)\cdot k + 4k = k^2 + 3k$ grid points. 
% \end{proof}






==> Approx2.tex <==

  Given a polygon $\mathcal P$, we will always assume that all its vertices are given by \emph{positive} integers in binary. We denote by $M$ the largest appearing integer and 
  we denote by $\diam(\P)$ the largest distance between 
  any two points in \P. Note that $\diam(\P)< 2 M$.
  We denote $L = 20 M > 10 $. Note that $\log L$ is linear in the input size.
  As a preprocessing step, we multiply all coordinates with $m = 2^{\lceil \log n \rceil} $. This takes at most $O(n \log n)$ time and ensures $n < L$.
  
  We define the grid $\Gamma$ as $(L^{-41}\cdot \mathbb{Z}^2) \cap \mathcal{P}$. Note that all vertices of $\mathcal P$ have integer coordinates and thus are included in $\Gamma$. We denote by $OPT$ an optimal solution to the \pgag problem and by $k$ its size.
  We denote by $OPT_\textup{grid}$ an optimal solution to the \textsc{Grid Guard Art Gallery Problem}, this is, guards are restricted to lie on the grid $\Gamma$, and denote by $k_\textup{grid}= |OPT_{grid}|$.


The idea is to show that the algorithm of Efrat and Har-Peled gives an approximation algorithm under the integer vertex representation assumption and the grid $\Gamma$ as described above.

\begin{theorem}[Efrat, Har-Peled~\cite{DBLP:journals/ipl/EfratH06}]
  Given a simple polygon $\mathcal P$ with $n$ vertices, one can spread a grid $\Gamma$ inside $\mathcal P$ , and compute an $O(\log k_\textup{grid})$-approximation to the smallest subset of $\Gamma$ that sees $\mathcal P$. The expected running time of the algorithm is $O(n \, k_\textup{grid}^2  \log  k_{grid} \, \log( n k_\textup{grid}) $ $  \, \log^2 \Delta)$,
  where $\Delta$ is the ratio between the diameter of the polygon and the grid size.
\end{theorem}
Note that the grid size equals $w = L^{-41}$, thus $\Delta \leq L^{42}$ and consequently $\log \Delta \leq 42 \log L$, which is polynomial in the size of the input. 

Efrat and Har-Peled implicitly use the real-RAM as model of computation. This is elementary computations are expected to take $O(1)$ time and coordinates of points are given by real numbers.
As we assume that coordinates are given by integers the word-RAM or integer-RAM is a more appropriate model of computation. All we need to know about this model is that we can upper bound the time for elementary computations polynomially by the bit-length of the involved numbers.
Thus going from the real-RAM to the word-RAM only adds a polynomial factor in 


It remains to show the following lemma.




==> AugmentedVisibility.tex <==
\subsection{Augmented Visibility}
 We are often not just in the case that the 
 local visibility property holds. But  $\grid(x)$
 can often see even more than $x$ itself, see
 Figure~\ref{fig:ConesContainment}.
 We call this loosely speaking the augmented visibility.
 In this section, we establish lower bounds on 
 the augmented visibility. Here, we are in 
 the unfortunate situation that we have to treat the 
 interior case and the boundary case differently.
 In the interior case, we will use that the 
 distance between  $\grid(x)$ and $x$ is at least 
 $\alpha/2$ under orthogonal projection to any line $\ell$.
 In the boundary and corner case we need to use additionally 
 the fact that  the distance between any 
 vertex $v$ and any supporting line not 
 containing $v$ is at least $1/L$, see Lemma~\ref{lem:distances} Item~\ref{itm:VertexLine}.
 
 \begin{restatable}[Augmenting Visibility]{lem}{AugmentedVisibility}
    \label{lem:AugmentedVisibility}
    Let $x , a \in \P$ and $r$ some reflex vertex.
  We make the following assumptions:
  \begin{enumerate}
   \item Width of  $\cone(x)$ larger than $\alpha L^{2}$.
   \item $D = \dist(a,r)\geq L^{-2}$.
   \item $d = \dist(a,\cone(x))\leq \alpha L^{-5}$.
   \item 
   \label{Cond:SuppLine}
   $\dist(a,\ell)\leq d$, for all supporting lines $\ell$.
  \end{enumerate}
  Then $\grid(x)$ sees $a$.
  \end{restatable}
 
 The proof will be given at the end of the section, when all 
 necessary lemmas and definitions are given.
 
  \begin{definition}[Left Reflex Vertex / Right Reflex Vertex]
    Given a point $x\in \P$ and a reflex vertex $r$ (not necessarily visible  
    from $x$).
    We define $\ell^L$ as the half-plane bounded by $\ell(x,r)$
    to the left of $\ell(x,r)$.
    And $\ell^R$ as the other half-plane bounded by $\ell(x,r)$.
    We say that $r$ is a \emph{left  reflex vertex}
    of $x$ if $\disk(r,\varepsilon)\cap \ell^{R} \subset \P$, for some $\varepsilon>0$.
    We say that $r$ is a \emph{right  reflex vertex}
    of $x$ if $\disk(r,\varepsilon)\cap \ell^{L} \subset \P$, for some $\varepsilon>0$.
 \end{definition}
 
 
 \begin{figure}[hbtp]
  \centering
 \includegraphics{AugmentingAngleDefinition}
 \caption{The point $x$ has $r$ as a right reflex vertex 
    and the augmenting angle equals $\beta$.}
 \label{fig:AugmentingAngleDefinition}
\end{figure}
 
 %\till{This must be specified for bad regions of the supporting line of the cone ..... }
 
 \begin{lemma}[Mutual Visibility]\label{lem:MutualVisibility}
  Given a point $x\in \P$ 
  and a left (right) reflex vertex $r$.
  Assume that $x$ is not in any $s$-bad region with respect to
  $r$ with $s\leq L \alpha$. Further let $g\in \grid(x)$
  on the right (left) of $\ell(x,r)$.
  Then holds that $g$ sees $r$.  
 \end{lemma}
 \begin{proof}
  See Figure~\ref{fig:MutualVisibility} for an illustration of this proof.
  In case that there is part of $\partial\P$ that blocks the visibility
  of $g$ there must exist a vertex $q$ in the triangle $\Delta(x,r,g)$.
  We will show that $x$ lies in an $s$-bad region of $r$ and $q$ with 
  $s = L \alpha$, which contradicts the assumption in the lemma.
  Denote with $c$ the distance between $x$ and $\ell(r,q)$ and by
  $p$ the orthogonal projection of $x$ onto $\ell(q,r)$. We denote by 
  $d = \dist(p,q)$. 
  At last we denote by $\beta$ the angle between $\seg(q,x)$ and $\ell(q,r)$. It is sufficient to show $\tan(\beta) < s$.
  Note that $\tan(\beta) = \frac{c}{d} \leq \frac{\alpha}{L^{-1}} = \alpha L$.
 \end{proof}

 
 \begin{figure}[hbtp]
  \centering
 \includegraphics{MutualVisibility}
 \caption{}
 \label{fig:MutualVisibility}
\end{figure}

 
 \begin{definition}[Augmenting Angle]
    Given a point $x$ and a left reflex vertex $r$ of $x$.
    We define for all $g\in  \grid(x)$ the angle $\beta_g$
    as the angle formed by $\ell(x,r)$ and $\ell(g,r)$ at $r$.
    The \emph{augmenting angle} $\beta(x,r,\alpha)$ of $x$ and $r$ is defined as the maximum
    angle $\beta_g$ among all $g\in  \grid(x)$ to the right of $\ell(x,r)$.
    When $\alpha$ is clear from the context, we write $\beta(x,r)$ and suppress $\alpha$ in the notation.
    The \emph{augmenting angle} $\beta(x,r)$ is defined in a symmetric way for a right reflex vertex $r$.
 \end{definition}
 
 
 
 
 
 
 \begin{definition}[Projection Distance]
 Given a point $x$ and assume that we are in the interior case,
 as explained in Definition~\ref{def:SurroundingGrid}.
 We denote by $g_1,g_2,g_3$ the  $\grid(x)$ points corresponding to the vertices of $\Delta$, see Definition~\ref{def:SurroundingGrid}.
 Further, let $\ell$ be any line and $t_1,t_2,t_3$ be the orthogonal 
 projections of $g_1,g_2,g_3$ onto $\ell$ and $x'$ be the projection
 of $x$, see Figure~\ref{fig:GridTriangleProjection}.
%  Without loss of generality the order along $\ell$ is $t_1,t_2,x', t_3$ (otherwise change the orientation of $\ell$.).
  Let $t_l$ be the left most and $t_r$ be the right most projected point on $\ell$.
 We define the \emph{projective distance} of $x$ to its 
 surrounding triangle with respect to $\ell$ as 
 \[\min (\dist(t_l,x'), \dist(x',t_r)).\]
 \end{definition}
 
 
 \begin{figure}[hbtp]
  \centering
 \includegraphics{GridTriangleProjection}
 \caption{}
 \label{fig:GridTriangleProjection}
\end{figure}
 
 \begin{lemma}[Large Distance in Projection]\label{lem:ProjectionDistance}
    In the interior case the projective 
    distance of $x$ is at least $\alpha/2$.
 \end{lemma}
 \begin{proof}
    Without loss of generality we  assume that $\ell$ contains $x$.
    Let us mentally rotate $\ell$ around $x$ and let us keep track of 
    $d_1 = \dist(x',t_1)$ and $d_2 = \dist(x',t_2)$, as indicated in Figure~\ref{fig:GridTriangleProjection}. It is easy to see that
    while $d_1$ decreases, $d_2$ increases. For reasons of symmetry,
    $\max(d_1,d_2)$ is minimized when  $d_1 = d_2$.
    In this case holds $d_1 = \cos( 60^{\circ})\, \alpha = \alpha/2$.
 \end{proof}



 \begin{figure}[hbtp]
  \centering
 \includegraphics{AugmentingAngle}
 \caption{}
 \label{fig:AugmentingAngle}
\end{figure}
 
 
 \begin{lemma}[Big Angle Interior]\label{lem:BigAngleInterior}
    Let $x\in \P$  in the interior case and $r$ 
    a left reflex vertex of $x$. 
    Assume that every point in  $\grid(x)$ sees 
    $r$. Then holds  $\tan(\beta(x,r)) \geq \frac{\alpha}{L}$
 \end{lemma}
 \begin{proof}
    Let $g$ be the surrounding grid point realizing the augmenting angle and $\ell$ be the line containing $g$ orthogonal to $\ell(x,r)$, as in Figure~\ref{fig:AugmentingAngle}.
    We denote by $p$ the intersection of $\ell$ and $\ell(x,r)$.
    Note that $\dist(g,p) \geq \alpha/2$, by Lemma~\ref{lem:ProjectionDistance}.
    Then holds 
    \[\tan(\beta) 
    = \frac{\dist(g,p)}{\dist(p,r)} 
    \geq \frac{\alpha/2}{\diam(\P)}
    \geq \frac{\alpha/2}{L/2} 
    = \frac{\alpha}{L}. \qedhere\]
 \end{proof}

 
 
 \begin{figure}[hbtp]
  \centering
 \includegraphics{NoAugmentingAngleBoundary}
 \caption{}
 \label{fig:NoAugmentingAngleBoundary}
\end{figure}
 
Let us now consider the boundary and corner case. Note that we do not have the augmented visibility property in this case, see Figure~\ref{fig:NoAugmentingAngleBoundary}.
However, in this case $r_1$ and $r_2$ 
are on the supporting line
of the segment intersecting $\Delta$.
If we exclude this case, we get a useful lower bound on the 
augmenting angle.
Here we need to use the fact that 
the distance between any vertex and a line spanned
by two vertices of $P$ is at least $L^{-1}$.

\begin{figure}[hbtp]
  \centering
 \includegraphics{AugmentingAngleBoundary}
 \caption{}
 \label{fig:AugmentingAngleBoundary}
\end{figure}

 \begin{lemma}[Big Angle Boundary/Corner] \label{lem:BigAngleBoundary}
    Let $x\in \P$ in the boundary or corner case. 
    Denote by $\ell_1$ and $\ell_2$ the supporting lines
    of the segments intersecting $\Delta(x)$. 
    (Maybe there is only one such line.) 
    Further let $r$ be a reflex vertex that 
    is neither on $\ell_1$ nor on $\ell_2$ and sees $x$ and  $\grid(x)$.
    Then it holds  $\tan(\beta(x,r)) \geq \frac{\alpha}{L^3}$.
 \end{lemma}
  \begin{proof}
  By Lemma~\ref{lem:distances} Item~\ref{itm:VertexLine} holds that $\dist(r,\ell_i) \geq L^{-1}$, for $i = 1,2$.
  For the following description, we refer to Figure~\ref{fig:AugmentingAngleBoundary}.
  It is not clear that $r$ can see all 
  vertices of  $\grid(x)$, but $r$ 
  can see either both vertices on
  $\ell_1$ or both vertices on $\ell_2$. 
  We denote this line by $\ell$ and by $p$ 
  the orthogonal projection of $r$
  onto $\ell$.
  By $q$ we denote the intersection 
  point of $\ell(x,r)$ and $\ell$.
  We denote by $g$ the point of  $\grid(x)$ 
  on $\ell$ closest to $p$.
  Further we denote by $\gamma$ the angle at $g$ formed by the rays 
  $\ray(g,r)$ and $\ray(g,p)$.
  We denote by $\delta$ the angle at $q$ formed by the ray $\ray(q,r)$
  and $\ray(q,p)$. 
  We denote by $\beta$ the angle at $r$ formed by the ray $\ray(r,q)$
  and $\ray(r,g)$.
  We denote $h = \dist(r,p)$, $D = \dist(g,p)$ and $d = \dist(q,g)$.
  
  
  The following is easy to see 
  \[180^{\circ} - \delta - \beta = 180^{\circ} - \gamma
  \quad \Rightarrow \quad \beta = \gamma - \delta.\]
  Further we know
  \[\tan(\gamma) = \frac{h}{D}, \quad \tan(\delta) = \frac{h}{ d + D}. \]
  By the addition theorem we can conclude
  \[\tan(\beta ) = \tan(\gamma - \delta) = \frac{\tan(\gamma) - \tan(\delta)}{1 + \tan(\gamma)\,\tan(\delta)}  
  =\] \[ = \frac{(h/D) - (h/(d+D))}{1 + (h/D)\,(h/(d+D))} = \frac{hd}{D(d+D)}\frac{D(d+D)}{D(d+D) + h^2} = \frac{hd}{D(d+D) + h^2}.\]
  Note that 
  \[hd \geq \frac{1}{L} \frac{\alpha}{2} \geq \frac{\alpha }{2L}, 
  \quad D(d+D) \leq 2\, \diam^2 \quad \textrm{and} \quad
  h^2 \leq \diam^2.
  \]
  This implies 
  \[\tan(\beta )  \geq   \frac{\alpha}{2 L \, 3\diam^2} 
  \geq \frac{\alpha}{L^3}.  \qedhere\]
  \end{proof}
 
 
 
  
 \AugmentedVisibility*
 
 \begin{proof}
      We consider first the case that there exists no vertex $v$, with $\dist(x,v) \leq L^{-1}$.
      
      \begin{figure}[hbtp]
	\centering
	
	 \begin{minipage}[b]{\linewidth}
      \centering 
      \includegraphics{AugmentedVisibility}
      \subcaption{}
	\label{subfig:AugmentedVisibility1}
     \end{minipage} 
	
	\vspace{0.5cm}
	
	\begin{minipage}[b]{\linewidth}
      \centering 
      \includegraphics{AugmentedVisibility2}
      \subcaption{}
	\label{subfig:AugmentedVisibility2}
     \end{minipage}
	
	\vspace{0.5cm}
	
	
	\begin{minipage}[b]{\linewidth}
      \centering 
      \includegraphics{AugmentingNeedsSupport}
      \subcaption{}
	\label{subfig:AugmentingNeedsSupport}
     \end{minipage}
	
	
	\caption{}
      \label{fig:AugmentedVisibility}
      \end{figure}
      
      Let $r$ be the reflex vertex, which defines the ray of $\cone(x)$, which is closer to $a$. Without loss of generality,
      let $r$ be a left reflex vertex w.r.t. $x$.
      
      By Lemma~\ref{lem:ThinCones}, holds that if $x$ is in an 
      $s$-bad region then the width of $\cone(x)$ is globally bounded by $sL$. As we assume the width to be at least $\alpha L^{2}$, we conclude that $x$ is not in an $s$-bad region with
      $s\leq \alpha L$.
%       
      By Lemma~\ref{lem:MutualVisibility} holds that all $g\in\grid(x)$ on the right of $\ell(x,r)$ 
      see $r$.
% 
      Then by Lemma~\ref{lem:BigAngleInterior} and Lemma~\ref{lem:BigAngleBoundary}, it holds, for the augmenting angle $\beta = \beta(x,r)$,
      \[\tan(\beta) \geq \alpha L^{-3}.\]
      Denote by $g\in \grid(x)$ the grid point realizing this angle.
%       
      Consider the cone $C$ with apex $r$ bounded by $\ray(x,r)$ and $\ray(g,r)$. We will first show that $a\in C$. 
      But this does not imply yet that $g$ really sees $a$ as there might be another blocking vertex contained inside $C$.
      In that case we can just repeat the argument with that reflex vertex.
%       
%       Denote by $p$ the orthogonal projection of $a$ onto $\ell(x,r)$, denote $d = \dist(a,p)$ and denote $D=\dist(a,p)$.
      We have to show $\tan(\beta) \geq \frac{d}{D}$.
      This follows from 
      \[\tan(\beta) \geq \alpha L^{-3} = \frac{\alpha L^{-5}}{L^{-2}} \geq \frac{d}{D}.\]
%       
      Now, the only reason why $g$ does not see $a$ would be a reflex vertex $q \in C$  that blocks the visibility, see Figure~\ref{subfig:AugmentedVisibility2}. 
      If there is more than one such vertex, let $q$ be the last vertex, that is still visible, before $a$.
      In this case, there is an augmenting angle $\gamma$ at $q$ which has the property $\tan(\gamma) > \alpha L^{-3}$.
      and further holds $\dist(q,a) \geq L^{-2}$. Thus the same argument as before can be applied and $a$ is in some cone $C'$
      with apex $p = \ell(x,r)\cap \ell(g,q)$.
      As $q$ was the last blocking vertex $g$ sees indeed $a$.
      
    Next, we consider the case that there exists some vertex $v$ with $\dist(x,v)\leq L^{-1}$. 
    This immediately implies $v\in \grid^*(x)$.
    So far, we have not used Condition~\ref{Cond:SuppLine}. 
    Let us give a short example, why this condition is actually necessary. See Figure~\ref{subfig:AugmentingNeedsSupport}.
    Here, the cone of $x$ with respect to $v$ and $r$ is very large. Nevertheless, $g$ is blocked 
    by the edges incident to $v$. The visibility of $v$ on the other hand is blocked by $r$.
    To see that the other conditions are not sufficient, we show that $\dist(a,\cone(x))$ can be made arbitrarily small.
    First note that $a$ is not visible from $v$ as long as it is on the other side of the supporting line $\ell(v,r)$.
    Further, when $x$ is moved towards $v$ the cone of $x$ comes arbitrarily close to $\ell(v,r)$. 
    Thus also $\dist(a,\cone(x))$ can be made arbitrarily small.
     
    Condition~\ref{Cond:SuppLine} immediately implies that $a$ is on the same side of $\ell(v,r)$ as $\cone(x)$
    and thus seen from $v$.
 \end{proof}


==> ConeProperties.tex <==
\subsection{Cones}
In this subsection, we want to establish some basic relations between the width of a cone and whether or not its apex lies in a bad region. 
Roughly speaking, we want to establish the following facts:
If a point lies in a bad region, we can upper bound the width
of the corresponding cone.
Reversely, this implies that a cone with large width, has
its apex outside a bad region.
Another useful fact later is that thin cones are very close to theit supporting lines.

  
\begin{figure}[htbp]
  \centering
  \includegraphics{ConeWidth}
  \caption{}
  \label{fig:ConeWidth}
\end{figure}


\till{refine definition.}
\noindent \textbf{Cone width.}
Let  $\cone(x)$ be a cone  with respect to reflex vertices $r_1$ and $r_2$ and $a$ be any point in the plane. Then $\ell(r_1,r_2)$ is the \emph{supporting line of} $\cone(x)$.
We define the \emph{orthogonal width} of $\cone(x)$ at $a$ as 
$\text{length}(\ell \cap \cone(x))$, where  $ \ell$ is the unique line orthogonal to $\ell(r_1,r_2)\}$ through the point $a$.
We define the \emph{width} of a cone $C(x)$ as \[\min \{\, \text{length}(\ell \cap C(x)) : a \in \ell \,\}.\]
By definition is the orthogonal width of a cone larger than the ordinary width.






\begin{lemma}[Thin Cones]\label{lem:ThinCones}
  Let $\cone(x)$ be a cone with apex $x$ in some $s$-bad region. Then the width of $\cone(x)$ is globally bounded by $s\,L$. 
\end{lemma}
\begin{proof}
  Let $x$ be in a $s$-bad region as in Figure~\ref{fig:EvilCone}. 
  \begin{figure}[htbp]
  \centering
  \includegraphics{EvilCone}
  \caption{}
  \label{fig:EvilCone}
\end{figure}
  Let $\Delta$ be the triangle as 
  indicated in Figure~\ref{fig:EvilCone}, 
  with vertices $a,b$ and $r_1$. 
  We bound the width of $\cone(x)$ by  $\dist(a,b)$.
  The segment $seg(a,r_1)$ forms a slope of $s$, with the line of $\ell(r_1,r_2)$.
  Beyond $\seg(r_1,r_2)$, the cone is contained in $\Delta$. As the distance between $r_1$ and $b$ is at most $\diam$, the cone has a width of at most $s\,  \diam(\P) < s \, L$.
\end{proof}


\begin{lemma}[Distance Cone supporting Line]
\label{lem:DistanceConeSupportingLine}
  Let $\cone(x)$ be some cone with supporting line $\ell$, $b\in \cone(x)$ and denote by $d$ the orthogonal width of $\cone(x)$ at position $b$. 
  Then $\dist(b,\ell) \leq dL$.
\end{lemma}
\begin{proof}
  \begin{figure}[htbp]
  \centering
  \includegraphics{ThinConesCloseSupp}
  \caption{}
  \label{fig:ThinConesCloseSupp}
  \end{figure}
  See Figure~\ref{fig:ThinConesCloseSupp} and the notation therein. 
  We show the claim by showing $d+e \leq d L $.
  The line $\ell$ is the unique line parallel to $\ell(x,r_1)$ through point $B$.
  As $\ell$ and $\ell(x,r_1)$ are parallel we know by Thales Theorem:
  \[\frac{1}{L}\leq 
  \frac{\dist(r_1,D)}{L}  \leq
%   \frac{\dist(r_1,D)}{\dist(r_1,C)}  \leq
  \frac{\dist(r_1,D)}{\dist(r_1,C)} 
  = \frac{d}{d+e}.\] 
  For the first inequality see Lemma~\ref{lem:distances} Item~\ref{itm:VertexVertex}. The second inequality follows from the fact that $L$ is larger than the distance between any two points inside \P. 
  It follows immediately $d+e\leq d  L$.
\end{proof}


\begin{lemma}[Cone Area Bound]\label{lem:ConeAreaBound}
  Given a cone $\cone(x)$ with reflex vertices $r_1$ and $r_2$. Let $r_2$ be the reflex vertex further away from $x$ and let the width of $\cone(x)$ at $r_2$ be $\beta$.
  Then the width of $\cone(x)$ is globally bounded by $\beta L^2$.
\end{lemma}
\begin{proof}
  \begin{figure}[htbp]
  \centering
  \includegraphics{ConeAreaBound}
  \caption{}
  \label{fig:ConeAreaBound}
  \end{figure}
  For the case that $\beta \geq 1/10$ the lemma follows trivially from the fact that the width of $C(x)$ is bounded by $D \leq \tfrac{L}{10}$. In order for $\beta$ to be smaller than $\tfrac{1}{10}$ the point $x$ must be to the left of the line $\ell$ through $r_1$ orthogonal to $\ell(r_1,r_2)$.
  From now on we can assume $\dist(x,r_2)\geq 1$. 
%   We show first that the width of $C(x)$ is globally bounded by $\beta L$. This implies an area bound of $\beta L^2$ immediately. 
  Let $A$ and $B$ be the points where $C(x)$ is bounded by $\beta L$, as in Figure~\ref{fig:ConeAreaBound}.
  By Thales Theorem we can infer \[\frac{\dist(x,B)}{\dist(x,r_2)} = \frac{\beta L}{\beta} = L.\] This implies $\dist(x,B)\geq L$ and thus $B\notin \P$. Thus the width of $C(x)$ is globally bounded by $\beta L$.
\end{proof}

==> GeneralCase.tex <==
\subsection{The General Case}
% \newpage

\begin{proof}[Proof  Lemma~\ref{lem:GridReplacement} without general position Part I]
  Recall that we denote by $OPT$ an optimal solution.
 For every point $x\in OPT$, we add the four set $G_1(x),G_2(x),G_3(x),G_4(x) \subset \Gamma$ defined as follows.
 We set $\alpha_i = L^{-10 \, i}$ and $G_i = \alpha_i\textrm{-}\grid(x)$.
%  
 We denote $G(x) = G_1(x) \cup G_2(x) \cup G_3(x) \cup G_4(x)$
 and $G = \bigcup_{x\in OPT} G(x)$.
  As $|G(x)|\leq 25$ implies $|G| \leq 25 |OPT|$. 
 We will show that $G$ sees the entire polygon.
%  
 We set $s_i$ to $L^{-10 \, i + 2}$.
 Thus Lemma~\ref{lem:LocalVisibility} implies that every $x$ not in any 
 $s_4$-bad region has the $\alpha_4$-local visibility property.
 
 For the remainder, we will fix some point $x\in OPT$ 
 in side some $s_4$-bad region with respect to 
 reflex vertices $r_1$ and $r_2$.
 Then we cannot guarantee that $G(x)$ sees the cone of $x$ behind $\seg(r_1,r_2)$. Let $a\in \cone(x)$ be such a point. 
  We will show that $a$ is seen by some other point $g\in G(y)$, with $y\neq x$.
 
 We will assume $\dist(a,r) > L^{-2}$. We treat the other case in Part II.
 (In Part I only $G_1,G_2$ and $G_3$ are needed.)
 As $x$ is in a $s_4$-bad region, we know that the 
 width of $\cone(x)$ is at most $s_4\,L$, by 
 Lemma~\ref{lem:ThinCones}. Let $D = \disk(a,s_4L^4)$. 
 Then $\cone(x)$ does not cover $D$. 
 By Lemma~\ref{lem:distances} Item~\ref{itm:DiskSector} the area of $D\cap \P$
 is at least $s_4^2 L^6$. On the other hand $\cone(x)$ covers at most $\diam(D)\, \textrm{width}(\cone(x))\leq (2\,s_4\,L^4)\,(s_4\,L) \leq s_4^2 L ^6$.

  
  \begin{figure}[htbp]
  \centering
   \begin{minipage}[b]{.45\linewidth}
      \centering 
      \includegraphics{NewPoint}
      \subcaption{	}
	\label{fig:NewPoint}
     \end{minipage} 
     \hspace{0.5cm}
     \begin{minipage}[b]{.45\linewidth}
      \centering 
      \includegraphics{NewSmallCone}
      \subcaption{}
	\label{fig:NewSmallCone}
     \end{minipage} 
  \caption{}
  \end{figure}
 
 Let $\cone(y)$ be the visibility cones covering $b$ with width $\beta$.
 (obviously $x\neq y$). 
 We consider two cases. 
 Case $1$:  $\beta > 4 \alpha_{3}L^2$.
 Case $2$: $\beta \leq 4 \alpha_{3}L^2$. 
 
 In case $1$, $y$ is not in an $s_3$-bad region with respect to its cone $\cone(y)$, by Lemma~\ref{lem:ThinCones}. (It might be in some bad region with respect to some other pair of opposite reflex vertices, but we don't car about that.)
 By Lemma~\ref{lem:AugmentingVisibility}, $G_3(y)$   sees $a$ as $\dist(a,\cone(y))\leq \alpha_4\,L^4 \leq \frac{\alpha_{3}}{10 L^2}$.
 
 
 In case $2$, All cones have width $\beta_j \leq 4 w_{3}L^2$. 
 This implies $\dist(a,l_i)\leq \dist(a,b_i) + \dist(b_i,l_i) \leq 10w_4 L^2 + 4w_{3}L^2 L \leq 5 w_{3}L^3$, for all $i$. Here we used Lemma~\ref{lem:DistanceConeSupportingLine}.
 Further $\dist(a,\ell)\leq 4w_4 L^2$ by Lemma~\ref{lem:ThinCones} and Lemma~\ref{lem:DistanceConeSupportingLine}.
 By Lemma~\ref{lem:distances} Item~\ref{itm:LinesCommonIntersection} all the supporting lines $\ell$ and $\ell_1,\ldots, \ell_t$ intersect in a point $p$ with $\dist(a,p)\leq 10 w_{3}L^3 \cdot L^2 = 10 w_{3}L^5$.
 From the assumption, $\dist(a,r) > L^{-2}$ for all reflex vertices $r$, follows
 $p$ is not a reflex vertex. To see this note $\dist(p,r) \geq \dist(r,a) - \dist(a,p) \geq L^{-2} - 10 w_{3}L^5 >0$.
 As $p$ is not a reflex vertex, non of the cones sees $p$, as $p$ is on the supporting line of all the cones.
 Thus, there is some cone $C(y)$ that covers $p$ with supporting line $\ell_y$. 
 
 
 By Lemma~\ref{lem:distances} Item~\ref{itm:IntersectionLine}, we know $\dist(p,\ell_y) \geq L^{-5}$. Using Lemma~\ref{lem:DistanceConeSupportingLine}, the width $\beta$ of $C(y)$ at position $p$ is at least $L^{-4}>4w_{2}L^2$.
 By Lemma~\ref{lem:ThinCones}, $y$ is not in a $2$-bad region and by Lemma~\ref{lem:AugmentingVisibility} the $G_2$ of $y$ see $a$, as $\dist(a,C(y)) \leq \dist(a,p) \leq 10 w_{3}L^5 < w_{2}/10L^{2}$.
\end{proof}

We postpone the proof of Part II, till all necessary technical lemmas and definitions are presented.


\noindent {\bf Up and Down reflex vertices}
\till{define up and down reflex vertices.}

\till{define left and right cones of a reflex vertex on a line.}

\till{for small cones orthogonal width and proper width are almost the same.}








\begin{lemma}[Small Left and Right Cones]
  Let $r$ be a reflex vertex on line $\ell$ with both neighbors $u,v$ of $r$ contained in the halfplane  $\ell^+$. 
  Further, assume that there are left and right cones of $r$ denoted by $C(x_1),\ldots ,C(x_t)$ all with width bounded by $\beta$ and $t\leq n$. Then the half-disk $d = \disk(r,\beta L^{3})\cap \ell^{-}$ is \emph{not} fully covered by the cones.
\end{lemma}
\begin{proof}
 The area of $d$ equals $\tfrac{\pi}{2} \beta^2 L^{6}$.
 The width of each cone $C(x_i)$ is globally bounded by $\beta L$ and thus the area $C(x_i)\cap d$ is bounded by $\beta L \cdot 2 \beta L^{3} = 2 \beta^{2} L^4$. Thus the area of all the cones inside $d$ is bounded by $n \cdot 2 \beta^{2} L^4 <  \tfrac{\pi}{2} \beta^2 L^{6}$.
\end{proof}





\begin{lemma}[Large Left and Right Cones]
  Let $r$ be a reflex vertex on line $\ell$ with both neighbors $u,v$ of $r$ contained in the halfplane  $\ell^+$. 
  Further, assume that there is one left and one right cone of $r$ denoted by $C(x)$ and $C(y)$ both of width at least $\beta$. Then the half-disk $d = \disk(r,\beta)\cap \ell^{-}$ \emph{is fully} covered by the cones.
\end{lemma}
\begin{proof}
\begin{figure}[htbp]
  \centering
  \includegraphics{LargeLeftAndRightCones}
  \caption{}
  \label{fig:LargeLeftAndRightCones}
\end{figure}
For the following refer to Figure~\ref{fig:LargeLeftAndRightCones}.
Consider the left cone $C(x)$ bounded by the reflex vertices $\overline{r}$ and $r$.
Note that the set $C(x)\cap \disk(r,\beta)$ is a half disk $d_x$ contained in $C(x)$. In other words the circle $C$ around $r$ with radius $\beta$ is not intersected by $\ray(x,r)$ as the width of $C(x)$ at $r$ is $\beta$.
Similarly, we define $d_y = C(y)\cap \disk(r,\beta)$. 
We show $d \subset d_1\cup d_2 $. As $d_1$ and $d_2$ are half disks with the same center $d_1\cup d_2$ form a disksector $s$. Note that $s$ contains some part of $\ell$ to the left and to the right of $r$. Further $s$ does not contain the segment $\seg(r,u)$. Thus $s$ contains $d$ as claimed.
\end{proof}



\till{Proof that there is a point close $a$ on $\ell$ not seen by left and right reflex vertices.}



\begin{proof}[Proof Lemma~\ref{lem:GridReplacement} Part II]
  Recall that we considered the situation that $x$ is in some $4$-bad region with respect to the reflex vertices $r_1$ and $r_2$ and that $a$ is a point in the cone $C(x)$. We denote $\ell = \ell(r_1,r_2)$.
  Here, we consider the case that there exists a reflex vertex $r$ such that $\dist(r,a)\leq L^{-2}$. As the distance between any two reflex vertices is at least one, there is at most one such $r$. Further $r$ needs to be on $\ell$. 
  To see this note the width of $C(x)$ is globally bounded by $4w_4L^2$ be Lemma~\ref{lem:ThinCones}. This implies $\dist(a,\ell)\leq 4w_4L^3$ by Lemma~\ref{lem:DistanceConeSupportingLine}. Let $\overline{r}\notin \ell$ be some reflex vertex. Then by Lemma~\ref{lem:distances} Item~\ref{itm:VertexLine} holds $\dist(\ell, \overline{r})\geq L^{-1}$. This implies $\dist(a,\overline{r})\geq  \dist(\ell,\overline{r}) - \dist(a,\ell)  \geq L^{-1} - 4w_4L^3 \gg L^{-2}$. But we assumed $\dist(a,r) \leq L^{-2}$.
  
  There are at least $2$ reflex vertices under consideration. See Figure~\ref{fig:ReflexVerticesOnL}.
%   
\begin{figure}[htbp]
  \centering
  \includegraphics{ReflexVerticesOnL}
  \caption{}
  \label{fig:ReflexVerticesOnL}
\end{figure}
% 
Let $r_1,\ldots,r_t$ be the reflex vertices on $\ell$, as indicated in Figure~\ref{fig:ReflexVerticesOnL}. In case that $a$ is in the vicinity of $r_1$ note that $a$ is seen by $G_4$ despite the fact that the local visibility property does not hold. 

\till{How to handle the upward reflex vertex $r_t$?}

Now, we consider the case that $a$ is in the vicinity of some downward reflex vertex, denoted by $r$. 
We distinguish two cases:
Case 1: Either all left cones or all right cones of $r$ have width at most $w_2$.
Case 2: There is at least one left and one right cone of $r$ with width at least $w_2$.

In case $1$ the proof works as in Part I. (Need to be a little careful with the existence of a cone that sees $p$. + disk around $a$ might not work as desired.
Pick a point on $\ell$ instead.)

In case $2$ we have some lower bound on the distance of $a$ and $r$ in terms of $w_3$. In case $2a)$, everything is fine anyway. (One large cone next to $a$.)

In case $2b)$ all cones next to $a$ are small. There is a point of intersection $p$ close to $a$.
Thus, $a$ is very close to $p$ in terms of $w_3$. 
This implies $p
\neq r$ and the proof follows as before.
\end{proof}



==> hardness.tex <==
Given a finite totally ordered set $Y=\{y_1, \ldots, y_{|Y|}\}$ (that is, for any $i, j \in [|Y|]$, $y_i \leq y_j$ iff $i \leqslant j$), a subset $S \subseteq Y$ is a \emph{$Y$-interval} if $S=\{y $ $|$ $ y_i \leq y \leq y_j\}$ for some $i$ and $j$.
We may denote by $\leq_Y$ the order of $Y$.
If $x$ is an element of a totally ordered set $Y$, $\ord(x)$ denotes the position of $x$ along this order, where $\ord$ of the first element is $0$, for notational convenience. 
The elements of a $Y$-interval are said to be \emph{consecutive along $\leq_Y$}.
A set-system $(X,\mathcal S)$ is said \emph{\sti} if $X$ can be partitioned into two totally ordered sets $A=\{a_1, \ldots, a_{|A|}\}$ and $B=\{b_1, \ldots, b_{|B|}\}$ such that each set $S \in \mathcal S$ is the union of an $A$-interval with a $B$-interval.

\begin{theorem}\label{thm:2-intervals-cover}
\ksc restricted to \sti instances with $N$ elements and $M$ sets is \wone-hard, and not solvable in time $(N+M)^{o(k / \log k)}$, unless the ETH fails.
\end{theorem}

% \appendixproof{\autoref{thm:2-intervals-cover}}
% {
\begin{proof}
We reduce from \mkc which remains \wone-hard when each color class has the same number $t$ of vertices. 
Let $G=(V=V_1 \cup \ldots \cup V_k, E)$ be an instance of \mkc such that $\forall i \in [k]$, $V_i=\{v^i_1, \ldots, v^i_t\}$, $m=|E|$, and $n=|V|=tk$.
For each pair $i < j \in [k]$, $E_{ij}$ denotes the set of edges $E(V_i,V_j)$ between $V_i$ and $V_j$.
For each $E_{ij}$ we give an arbitrary order to the edges: $e^{ij}_1, \ldots, e^{ij}_{|E_{ij}|}$.
We build an equivalent instance $(X, \mathcal S)$ of \ksc with $4{k \choose 2}+4m+tk(k+1)+4k$ elements and $4m+2kt$ sets, and such that $(X, \mathcal S)$ is \sti.
We call $A$ and $B$ the two sets of the partition of $X$ that realizes that $(X, \mathcal S)$ is \sti.

For each of the color class $V_i$, we add $tk+2$ elements to $A$ with the following order: $x_b(i), x(i,1,1), \ldots, $ $x(i,1,t), x(i,2,1), \ldots, x(i,2,t), \ldots, x(i,i-1,1), \ldots, $ $x(i,i-1,t), x(i,i+1,1), \ldots,$ $x(i,i+1,t), \ldots, x(i,k+1,1), \ldots, x(i,k+1,t),  x_e(i)$, and call $X(i)$ the set containing those elements.
We also denote by $X(i,j)$ the set $\{x(i,j,1), x(i,j,2), \ldots, x(i,j,t)\}$ (hence, $X(i)=\bigcup_{j \neq i}X(i,j) \cup \{x_b(i),x_e(i)\}$).
For each $E_{ij}$, we add $3|E_{ij}|+2$ elements to $B$ with the order: $y_b(i,j), y(i,j,1), \ldots, $ $y(i,j,3|E_{ij}|), y_e(i,j)$, and denote by $Y(i,j)$ the set containing them.
For each pair $i < j \in [k]$ and for each edge $e^{ij}_c=v^i_av^j_b$ in $E_{ij}$ (with $a, b \in [t]$ and $c \in [|E_{ij}|]$), we add to $\mathcal S$ the two sets $S(e^{ij}_c,v^i_a)=\{x(i,j,a), x(i,j,a+1), \ldots, x(i,j,t),$ $x(i,j+1,1), \ldots, x(i,j+1,a-1)\} \cup \{y(i,j,c),$ $\ldots, y(i,j,c+|E_{ij}|-1)\}$ and $S(e^{ij}_c,v^j_b)=\{x(j,i,b), x(j,i,b+1), \ldots, x(j,i,t),$ $ x(j,i+1,1), \ldots x(j,i+1,b-1)\} \cup \{y(i,j,c+|E_{ij}|), \ldots, y(i,j,c+2|E_{ij}|-1)\}$.
Observe that in case $j=i+1$, then all the elements of the form $x(j,i+1,\cdot)$ in set $S(e^{ij}_c,v^j_b)$ are in fact of the form $x(j,i+2,\cdot)$.
We may also notice that in case $a=1$ (resp. $b=1$), then there is no element of the form $x(i,j+1,\cdot)$ (resp. $x(j,i+1,\cdot)$) in set $S(e^{ij}_c,v^i_a)$ (resp. in set $S(e^{ij}_c,v^j_b)$).
For each pair $i < j \in [k]$, we also add to $A$ the $|E_{ij}|+2$ elements of a set $Z(i,j)$ ordered: $z_b(i,j), z(i,j,1), \ldots, z(i,j,|E_{ij}|), z_e(i,j)$, and for each edge $e^{ij}_c$ in $E_{ij}$ (with $c \in [|E_{ij}|]$), we add to $\mathcal S$ the two sets $S(e^{ij}_c,\vdash)=\{z_b(i,j), z(i,j,1), \ldots, z(i,j,|E_{ij}|-c\} \cup \{y_b(i,j), y(i,j,1) \ldots y(i,j,c-1)\}$ and $S(e^{ij}_c,\dashv)=\{z(i,j,|E_{ij}|-c+1),$ $\ldots, z(i,j,|E_{ij}|, z_e(i,j)\} \cup \{y(i,j,c+2|E_{ij}|) \ldots y(i,j,3|E_{ij}|), y_e(i,j)\}$.
Finally, for each $i \in [k]$, we add to $B$ the $t+2$ elements of a set $W(i)$ ordered: $w_b(i), w(i,1), \ldots, $ $w(i,t),$ $w_e(i)$, and for all $a \in [t]$, we add the sets $S(i,a,\vdash)=\{x_b(i), x(i,1,1), \ldots, x(i,1,a-1)\}$ $\cup \{w_b(i), w(i,1), \ldots, w(i,t-a+1)\}$ and $S(i,a,\dashv)$ $=\{x(i,k+1,a), \ldots, x(i,k+1,t), x_e(i)\} \cup \{w(i,t-a+2), \ldots, w(i,t), w_e(i)\}$.

No matter the order in which we put the $X(i)$'s and $Z(i,j)$'s in $A$ (respectively the $Y(i,j)$'s and $W(i)$'s in $B$), the sets we defined are all unions of an $A$-interval with a $B$-interval, provided we keep the elements within each $X(i)$, $Z(i,j)$, $Y(i,j)$, and $W(i)$ consecutive (and naturally, in the order we specified).
Though, to clarify the construction, we fix the following order: $X(1), X(2), \ldots, X(k), Z(1,2), Z(1,3), \ldots, Z(1,k), Z(2,3), \ldots, Z(2,k), \ldots, $ $Z(k-2,k-1), Z(k-2,k), Z(k-1,k)$ for $A$ and $Y(1,2), Y(1,3), \ldots, Y(1,k), Y(2,3), \ldots,$ $Y(2,k), \ldots, Y(k-2,k-1), Y(k-2,k), Y(k-1,k), W(1), W(2), \ldots, W(k)$ for $B$.
We ask for a set cover with $2k^2$ sets.
This ends the construction (see Figure~\ref{fig:set-cover-2-block} for an illustration of the construction for the instance graph of Figure~\ref{fig:instance-of-mkc}).

\begin{figure}
\centering
\begin{tikzpicture}
\node (tv1) at (1,1.6) {$G$} ;

\node[draw,circle,inner sep=0.01cm] (v11) at (0,0) {$v^1_1$} ;
\node[very thick,draw,circle,inner sep=0.01cm] (v12) at (0,1) {$v^1_2$} ;
\node[draw, rectangle, rounded corners, fit=(v11) (v12)] (V1) {} ;
\node (tv1) at (0,-0.6) {$V_1$} ;

\node[draw,circle,inner sep=0.01cm] (v21) at (1,0) {$v^2_1$} ;
\node[very thick,draw,circle,inner sep=0.01cm] (v22) at (1,1) {$v^2_2$} ;
\node[draw, rectangle, rounded corners, fit=(v21) (v22)] (V2) {} ;
\node (tv2) at (1,-0.6) {$V_2$} ;

\node[draw,circle,inner sep=0.01cm] (v31) at (2,0) {$v^3_1$} ;
\node[draw,circle,inner sep=0.01cm] (v32) at (2,1) {$v^3_2$} ;
\node[draw, rectangle, rounded corners, fit=(v31) (v32)] (V3) {} ;
\node (tv3) at (2,-0.6) {$V_3$} ;

\draw (v11) -- (v22) ;
\draw (v11) -- (v32) ;
\draw (v21) -- (v31) ;
\draw[very thick] (v12) -- (v22) ;
\draw (v12) -- (v31) ;
\draw (v22) -- (v31) ;
\draw[very thick] (v12) -- ($(v31)!1cm!(v12)$) ;
\draw[very thick] (v22) -- ($(v31)!0.7cm!(v22)$) ;
\end{tikzpicture}
\caption{A simple instance of \mkc. The elements in bold: vertices $v^1_2$ and $v^2_2$, edge $v^1_2v^2_2$, and half of the edges $v^1_2v^3_1$ and $v^2_2v^3_1$ correspond to the selection of sets depicted in Figure~\ref{fig:set-cover-2-block}.}
\label{fig:instance-of-mkc}
\end{figure}

\begin{figure}
%\resizebox{100pt}{100pt}
\setlength{\tabcolsep}{0.2pt}
%\small{
%\rot{
\resizebox{\columnwidth}{!}
{
\begin{tabular}{ccccccccc|cccccccc|c|cccc|c||cccccccc|c|cccc|cccc|cc}

& \rot{$x_b(1)$} & \rot{$x(1,2,1)$} & \rot{$x(1,2,2)$} & \rot{$x(1,3,1)$} & \rot{$x(1,3,2)$} & \rot{$x(1,4,1)$} & \rot{$x(1,4,2)$} & \rot{$x_e(1)$} & \rot{$x_b(2)$} & \rot{$x(2,1,1)$} & \rot{$x(2,1,2)$} & \rot{$x(2,3,1)$} & \rot{$x(2,3,2)$} & \rot{$x(2,4,1)$} & \rot{$x(2,4,2)$} & \rot{$x_e(2)$} & $\ldots$ & \rot{$z_b(1,2)$} & \rot{$z(1,2,1)$} & \rot{$z(1,2,2)$} & \rot{$z_e(1,2)$} & $\ldots$ & \rot{$y_b(1,2)$} & \rot{$y(1,2,1)$} & \rot{$y(1,2,2)$} & \rot{$y(1,2,3)$} & \rot{$y(1,2,4)$} & \rot{$y(1,2,5)$} & \rot{$y(1,2,6)$} & \rot{$y_e(1,2)$} & $\ldots$ & \rot{$w_b(1)$} & \rot{$w(1,1)$} & \rot{$w(1,2)$} & \rot{$w_e(1)$} & \rot{$w_b(2)$} & \rot{$w(2,1)$} & \rot{$w(2,2)$} & \rot{$w_e(2)$} & $\ldots$ \\
$S(1,1,\vdash)$ & 1 & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & 1 & 1 & 1 & & & & & & & \\
$\mathbf{S(1,2,\vdash)}$ & \textbf{1} & \textbf{1} & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & \textbf{1} & \textbf{1} & & & & & & & & \\
$S(v^1_1v^2_2,v^1_1)$ & & 1 & 1 & & & & & & & & & & & & & & & & & & & & & 1 & 1 & & & & & & & & & & & & & & &  \\
$\mathbf{S(v^1_2v^2_2,v^1_2)}$ & & & \textbf{1} & \textbf{1} & & & & & & & & & & & & & & & & & & & & &\textbf{1} & \textbf{1} & & & & & & & & & & & & & & \\
$S(v^1_1v^3_2,v^1_1)$ & & & & 1 & 1 & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & \\
$\mathbf{S(v^1_2v^3_1,v^1_2)}$ & & & & & \textbf{1} & \textbf{1} & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & &\\
$S(1,1,\dashv)$ & & & & & & 1 & 1 & 1 & & & & & & & & & & & & & & & & & & & & & & & & & & & 1 & & & &\\
$\mathbf{S(1,2,\dashv)}$ & & & & & & & \textbf{1} & \textbf{1} & & & & & & & & & & & & & & & & & & & & & & & & & & \textbf{1} & \textbf{1} & & & &\\
\hline
$S(2,1,\vdash)$ & & & & & & & & & 1 & & & & & & & & & & & & & & & & & & & & & & & & & & & 1 & 1 & 1 & & \\
$\mathbf{S(2,2,\vdash)}$ & & & & & & & & & \textbf{1} & \textbf{1} & & & & & & & & & & & & & & & & & & & & & & & & & & \textbf{1} & \textbf{1} & &  & & \\
$S(v^2_2v^1_1,v^2_2)$ & & & & & & & & & & & 1 & 1 & & & & & & & & & & & & & & 1 & 1 & & & & & & & & &  & & & &\\
$\mathbf{S(v^2_2v^1_2,v^2_2)}$ & & & & & & & & & & & \textbf{1} & \textbf{1} & & & & & & & & & & & & & & & \textbf{1} & \textbf{1} & & & & & & & & & & & \\
$S(v^2_1v^3_1,v^2_1)$ & & & & & & & & & & & & 1 & 1 & & & & & & & & & & & & & & & & & & & & & &  & & & &  \\
$\mathbf{S(v^2_2v^3_1,v^2_2)}$ & & & & & & & & & & & & & \textbf{1} & \textbf{1} & & & & & & & & & & & & & & & & & & & & & & & & &  \\
$S(2,1,\dashv)$ & & & & & & & & & & & & & & 1 & 1 & 1 & & & & & & & & & & & & & & & & & & & & & & & 1 \\
$\mathbf{S(2,2,\dashv)}$ & & & & & & & & & & & & & & & \textbf{1} & \textbf{1} & & & & & & & & & & & & & & & & & & & & & & \textbf{1} & \textbf{1} \\
\hline
$\mathbf{S(v^1_2v^2_2,\vdash)}$ & & & & & & & & & & & & & & & & & & \textbf{1} & & & & & \textbf{1} & \textbf{1} & & & & & & & & & & & & & & & & \\
$S(v^1_1v^2_2,\vdash)$ & & & & & & & & & & & & & & & & & & 1 & 1 & & & & 1 & & & & & & & & & & & & & & & & & & \\
$\mathbf{S(v^1_2v^2_2,\dashv)}$ & & & & & & & & & & & & & & & & & & & \textbf{1} & \textbf{1} & \textbf{1} & & & & & & & & \textbf{1} & \textbf{1} & & & & & &  & & & &\\
$S(v^1_1v^2_2,\dashv)$ & & & & & & & & & & & & & & & & & & & & 1 & 1 & & & & & & & 1 & 1 & 1 & & & & & & & & & &\\

%& \rot{$x_b(3)$} & \rot{$x(3,1,1)$} & \rot{$x(3,1,2)$} & \rot{$x(3,2,1)$} & \rot{$x(3,2,2)$} & \rot{$x_e(3)$} \\
\end{tabular}
}
\caption{The sets of $\mathcal S_b(1)$, $\mathcal S_b(2)$, $\mathcal S_e(1)$, $\mathcal S_e(2)$, $\mathcal S(1,2,\vdash)$, $\mathcal S(1,2,\dashv)$, $\mathcal S(1,2)$, $\mathcal S(2,1)$ for the graph of Figure~\ref{fig:instance-of-mkc}. The sets of $\mathcal S(1,3)$ and $\mathcal S(2,3)$ are also represented but only their part in $A$.}
\label{fig:set-cover-2-block}
\end{figure}


For each $i \in [k]$, let us denote by $\mathcal S_b(i)$ respectively $\mathcal S_e(i)$, all the sets in $\mathcal S$ that contains element $x_b(i)$, respectively $x_e(i)$.
For each pair $i \neq j \in [k]$, we denote by $\mathcal S(i,j)$ all the sets in $\mathcal S$ that contains element $x(i,j,t)$.
Finally, for each pair $i < j \in [k]$, we denote by $\mathcal S(i,j,\vdash)$, respectively $\mathcal S(i,j,\dashv)$, all the sets in $\mathcal S$ that contains element $y_b(i,j)$, respectively $y_e(i,j)$.
One can observe that the $\mathcal S_b(i)$'s, $\mathcal S_e(i)$'s, $\mathcal S(i,j)$'s, $\mathcal S(i,j,\vdash)$'s, and $\mathcal S(i,j,\dashv)$'s partition $\mathcal S$ into $k+k+k(k-1)+2{k \choose 2}=2k^2$ partite sets\footnote{We do not call them \emph{color classes} to avoid the confusion with the color classes of the instance of \mkc.}.
Thus, as each of the $2k^2$ partite sets $\mathcal S'$ has a private element which is only contained in sets of $\mathcal S'$, a solution has to contain one set in each partite set.

Assume there is a multicolored clique $\mathcal C = \{v^1_{a_1}, \ldots, v^k_{a_k}\}$ in $G$.
We show that $\mathcal T=\{S(v^i_{a_i}v^j_{a_j},v^i_{a_i}) $ $|$ $i < j \in [k]\} \cup \{S(v^i_{a_i}v^j_{a_j},v^j_{a_j}) $ $|$ $i < j \in [k]\} \cup \{S(i,a_i,\vdash) $ $|$ $i \in [k]\} \cup \{S(i,a_i,\dashv) $ $|$ $i \in [k]\}\cup \{S(v^i_{a_i}v^j_{a_j},\vdash)$ $|$ $i < j \in [k]\} \cup  \{S(v^i_{a_i}v^j_{a_j},\dashv)$ $|$ $i < j \in [k]\}$ is a set cover of $(\mathcal S,X)$ of size $2k^2$.
As $\mathcal C$ is a clique, $\mathcal T$ is well defined and it contains $2{k \choose 2}+2k+2{k \choose 2}=2k^2$ sets.
For each $i \in [k]$, the elements $x(i,1,a_i), \ldots, x(i,1,t), \ldots, x(i,k+1,1), \ldots, x(i,k+1,a_i-1)$ are covered by the sets $S(v^1_{a_1}v^i_{a_i},v^i_{a_i}), S(v^2_{a_2}v^i_{a_i},v^i_{a_i}), \ldots, S(v^i_{a_i}v^k_{a_k},v^i_{a_i})$.
Indeed, $S(v^j_{a_j}v^i_{a_i},v^i_{a_i})$ (or $S(v^i_{a_i}v^j_{a_j},v^i_{a_i})$ if $j > i$) covers all the elements $x(i,j,a_i), \ldots, x(i,j,t), x(i,j+1,1), \ldots, x(i,j+1,a_i-1)$ (again, in case $i+1 = j$, replace $\emph{j+1}$ by $\emph{i+1}$).
For each $i \in [k]$, the elements $x_b(i), x(i,1,1), \ldots, x(i,1,a_i-1), x(i,k+1,a_i), \ldots, x(i,k+1,t), x_e(i)$ and of $W(i)$ are covered by $S(i,a_i,\vdash)$ and $S(i,a_i,\dashv)$.
For all $i < j \in [k]$, say $v^i_{a_i}v^j_{a_j}$ is the $c$-th edge $e^{ij}_c$ in the arbitrary order of $E_{ij}$.
Then, the elements $y(i,j,c), y(i,j,c+1), \ldots, y(i,j,c+2|E_{ij}|-1)$ are covered by $S(v^i_{a_i}v^j_{a_j},v^i_{a_i})$ and $S(v^i_{a_i}v^j_{a_j},v^j_{a_j})$.
Finally, the elements $y_b(i,j), y(i,j,1), \ldots, y(i,j,c-1), y(i,j,$ $c+2|E_{ij}|), \ldots, y(i,j,3|E_{ij}|), y_e(i,j)$ and of $Z(i,j)$ are covered  by $S(v^i_{a_i}v^j_{a_j},\vdash)$ and $S(v^i_{a_i}v^j_{a_j},\dashv)$.

Assume now that the set-system $(X,\mathcal S)$ admits a set cover $\mathcal T$ of size $2k^2$.
As mentioned above, this solution $\mathcal T$ should contain exactly one set in each partite set (of the partition of $\mathcal S$).
For each $i \in [k]$, to cover all the elements of $W(i)$, one should take $S(i,a_i,\vdash)$ and $S(i,a'_i,\dashv)$ with $a_i \leqslant a'_i$.
Now, each set of $\mathcal S(i,j)$ has their $A$-intervals containing exactly $t$ elements.
This means that the only way of covering the $tk+2$ elements of $X(i)$ is to take $S(i,a_i,\vdash)$ and $S(i,a'_i,\dashv)$ with $a_i \geqslant a'_i$ (therefore $a_i=a'_i$), and to take all the $k-1$ sets of $\mathcal S(i,j)$ (for $j \in [k] \setminus \{i\}$) of the form $S(v^i_{a_i}v^j_{s_j},v^i_{a_i})$, for some $s_j \in [t]$.
So far, we showed that a potential solution of \ksc should stick to the same vertex $v^i_{a_i}$ in each \emph{color class}.
We now show that if one selects $S(v^i_{a_i}v^j_{s_j},v^i_{a_i})$, one should be consistent with this choice and also selects $S(v^i_{a_i}v^j_{s_j},v^j_{s_j})$.
In particular, it implies that, for each $i \in [k]$, $s_i$ should be equal to $a_i$.
For each $i \neq j \in [k]$, to cover all the elements of $Z(i,j)$, one should take $S(e^{ij}_{c_{ij}},\vdash)$ and $S(e^{ij}_{c'_{ij}},\dashv)$ with $c_{ij} \geqslant c'_{ij}$.
Now, each set of $\mathcal S(i,j)$ and each set of $\mathcal S(j,i)$ has their $B$-intervals containing exactly $|E_{ij}|$ elements.
This means that the only way of covering the $3|E_{ij}|+2$ elements of $Y(i,j)$ is to take $S(e^{ij}_{c_{ij}},\vdash)$ and $S(e^{ij}_{c'_{ij}},\dashv)$ with $c_{ij} \leqslant c'_{ij}$ (therefore, $c_{ij} = c'_{ij}$), and to take the sets $S(v^i_{a_i}v^j_{a_j},v^i_{a_i})$ and $S(v^i_{a_i}v^j_{a_j},v^j_{a_j})$.
Therefore, if there is a solution to the \ksc instance, then there is a multicolored clique $\{v^1_{a_1}, \ldots, v^k_{a_k}\}$ in $G$.

In this reduction, there is a quadratic blow-up of the parameter.
Under the ETH, it would only forbid, an algorithm solving \ksc on \sti instances in time $(N+M)^{o(\sqrt k)}$.
Marx showed that \textsc{Subgraph Isomorphism} cannot be solved in time $n^{o(k / \log k)}$ where $k$ is the number of edges of the pattern graph, under the ETH \cite{Marx10}.
Usually, this result enables to improve a lower bound obtained by a reduction from \mkc, from exponent $o(\sqrt k)$ to exponent $o(k / \log k)$, by doing more or less the same reduction but from \textsc{Multicolored Subgraph Isomorphism}.
As we shall see, \ksc on \sti instances is no exception to this rule of thumb.  
In the \textsc{Multicolored Subgraph Isomorphism} problem, one is given a graph with $n$ vertices partitioned into $l$ color classes $V_1, \ldots, V_l$ such that only $k$ of the ${l \choose 2}$ sets $E_{ij}=E(V_i,V_j)$ are non empty.
The goal is to pick one vertex in each color class so that the selected vertices induce $k$ edges.
The technique of color coding and the result of Marx \cite{Marx10} shows that, under the ETH, \textsc{Multicolored Subgraph Isomorphism} cannot be solved in time $n^{o(k / \log k)}$.
Naturally, this result still holds when restricted to connected input graphs.
In that case, $k \geqslant l-1$.
We can do the previous reduction from \textsc{Multicolored Subgraph Isomorphism} and suppress $X(i,j)$, $X(j,i)$, $Z(i,j)$, and $Y(i,j)$, and the sets defined over these elements, whenever $E_{ij}$ is empty.
We now ask for a set cover with $2l+4k \leqslant 6k+2$ sets.
One can check that the produced set cover instance is still \sti and that the way of proving correctness does not change.
Therefore, under the ETH, \ksc restricted to \sti instances cannot be solved in time $(N+M)^{o(k / \log k)}$.
\end{proof}
% }

In the \textsc{2-Track Hitting Set} problem, the input consists of an integer $k$, two totally ordered ground sets $A$ and $B$ of the same cardinality, and two sets $\mathcal S_A$ of $A$-intervals, and $\mathcal S_B$ of $B$-intervals. 
In addition, the elements of $A$ and $B$ are in one-to-one correspondence $\phi: A \rightarrow B$ and each pair $(a,\phi(a))$ is called a \emph{$2$-element}. 
The goal is to find, if possible, a set $S$ of $k$ $2$-elements such that the first projection of $S$ is a hitting set of $A$, and the second projection of $S$ is a hitting set of $B$.

\shs is the same problem with color classes over the $2$-elements, and a restriction on the one-to-one mapping $\phi$.
Given two integers $k$ and $t$, $A$ is partitioned into $(C_1,C_2,\ldots,C_k)$ where $C_j=\{a^j_1, a^j_2, \ldots, a^j_t\}$ for each $j \in [k]$.
$A$ is ordered: $a^1_1, a^1_2, \ldots, a^1_t, a^2_1, a^2_2, \ldots, a^2_t, \ldots, a^k_1, a^k_2, \ldots, a^k_t$.
We define $C'_j:=\phi(C_j)$ and $b^j_i := \phi(a^j_i)$ for all $i \in [t]$ and $j \in [k]$.
We now impose that $\phi$ is such that, for each $j \in [k]$, the $t$ elements of $C'_j$ are consecutive along $\leq_B$.
That is, $B$ is ordered: $C'_{\sigma(1)}, C'_{\sigma(2)}, \ldots, C'_{\sigma(k)}$ for some permutation on $[k]$, $\sigma \in \mathfrak S_k$.
For each $j \in [k]$, the order of the elements within $C'_j$ can be described by a permutation $\sigma_j \in \mathfrak S_t$ such that the ordering of $C'_j$ is: $b^j_{\sigma_j(1)}, b^j_{\sigma_j(2)}, \ldots, b^j_{\sigma_j(t)}$.
In what follows, it will be convenient to see an instance of \shs as a tuple $\mathcal I=(k \in \mathbb{N},t \in \mathbb{N}, \sigma \in \mathfrak S_k, \sigma_1 \in \mathfrak S_t, \ldots, \sigma_k \in \mathfrak S_t, \mathcal S_A, \mathcal S_B)$, where we recall that $\mathcal S_A$ is a set of $A$-intervals and $\mathcal S_B$ is a set of $B$-intervals.
We denote by $[a^j_i,a^{j'}_{i'}]$ (resp. $[b^j_i,b^{j'}_{i'}]$) all the elements $a \in A$ (resp. $b \in B$) such that $a^j_i \leq_A a \leq_A a^{j'}_{i'}$ (resp. $b^j_i \leq_B b \leq_B b^{j'}_{i'}$).

\begin{figure}
\centering
\begin{tikzpicture}

\definecolor{col1}{rgb}{1,0,0}
\definecolor{col2}{rgb}{0,1,0}
\definecolor{col3}{rgb}{0,0,1}
\definecolor{col4}{rgb}{1,1,0}
\def\p{-2}
\def\e{0.5}

\def\t{6}
\def\k{4}
\foreach \j [count = \ja from 0] in {1,...,\k}{
\foreach \i in {1,...,\t}{
\node (a\j\i) at (\e * \i + \e * \ja * \t, 0) {$a^\j_\i$} ;
}
\node[draw, fill=col\j, opacity=0.3, rectangle, rounded corners, thick, fit=(a\j1) (a\j\t),label=above:$C_\j$,inner sep=-0.05cm] (c\j) {} ;
}
\node[rectangle, rounded corners, thick, fit=(c1) (c\k),label=north:$A$,inner sep=0.4cm] (A) {} ;

\node (b34) at (\e, \p) {$b^3_4$} ;
\node (b32) at (2*\e, \p) {$b^3_2$} ;
\node (b33) at (3*\e, \p) {$b^3_3$} ;
\node (b36) at (4*\e, \p) {$b^3_6$} ;
\node (b31) at (5*\e, \p) {$b^3_1$} ;
\node (b35) at (6*\e, \p) {$b^3_5$} ;
\node[draw, fill=col3, opacity=0.3, rectangle, rounded corners, thick, fit=(b34) (b35),label=below:$C'_3$,inner sep=-0.05cm] (cp3) {} ;

\begin{scope}[xshift=6*\e cm]
\node (b12) at (\e, \p) {$b^1_2$} ;
\node (b14) at (2*\e, \p) {$b^1_4$} ;
\node (b11) at (3*\e, \p) {$b^1_1$} ;
\node (b15) at (4*\e, \p) {$b^1_5$} ;
\node (b16) at (5*\e, \p) {$b^1_6$} ;
\node (b13) at (6*\e, \p) {$b^1_3$} ;
\node[draw, fill=col1, opacity=0.3, rectangle, rounded corners, thick, fit=(b12) (b13),label=below:$C'_1$,inner sep=-0.05cm] (cp1) {} ;
\end{scope}

\begin{scope}[xshift=12*\e cm]
\node (b43) at (\e, \p) {$b^4_3$} ;
\node (b46) at (2*\e, \p) {$b^4_6$} ;
\node (b45) at (3*\e, \p) {$b^4_5$} ;
\node (b42) at (4*\e, \p) {$b^4_2$} ;
\node (b41) at (5*\e, \p) {$b^4_1$} ;
\node (b44) at (6*\e, \p) {$b^1_4$} ;
\node[draw, fill=col4, opacity=0.3, rectangle, rounded corners, thick, fit=(b43) (b44),label=below:$C'_4$,inner sep=-0.05cm] (cp4) {} ;
\end{scope}

\begin{scope}[xshift=18*\e cm]
\node (b21) at (\e, \p) {$b^2_1$} ;
\node (b25) at (2*\e, \p) {$b^2_5$} ;
\node (b22) at (3*\e, \p) {$b^2_2$} ;
\node (b24) at (4*\e, \p) {$b^2_4$} ;
\node (b26) at (5*\e, \p) {$b^2_6$} ;
\node (b23) at (6*\e, \p) {$b^2_3$} ;
\node[draw, fill=col2, opacity=0.3, rectangle, rounded corners, thick, fit=(b21) (b23),label=below:$C'_2$,inner sep=-0.05cm] (cp2) {} ;
\end{scope}

\node[rectangle, rounded corners, thick, fit=(cp3) (cp2),label=south:$B$,inner sep=0.4cm] (B) {} ;

\foreach \j in {1,...,\k}{
\draw[very thick,opacity=0.8] (c\j.south) -- (cp\j.north) ; 
}

\foreach \i in {1,...,\t}{
\draw (a1\i.south) -- (b1\i.north) ; 
}


\node (s) at (6.25,-1) {$\sigma$} ;
\node (s1) at (1.5,-1) {$\sigma_1$} ;

\node (oa) at (-0.1,0) {$\leq_A:$} ;
\node (ob) at (-0.1,-2) {$\leq_B:$} ;

\end{tikzpicture}
\caption{An illustration of the $k+1$ permutations $\sigma \in \mathfrak S_k$, $\sigma_1 \in \mathfrak S_t$, \dots, $\sigma_k \in \mathfrak S_t$ of an instance of \shs, with $k=4$ and $t=6$.}
\label{fig:permutations}
\end{figure}

\begin{corollary}\label{cor:main}
\shs is \wone-hard, and not solvable in time $|\mathcal I|^{o(k / \log k)}$, unless the ETH fails.
\end{corollary}

% \appendixproof{Corollary~\ref{cor:main}}
% {
\begin{proof}
This result is a consequence of Theorem~\ref{thm:2-intervals-cover}.
Let $(A \uplus B, \mathcal S)$ be a \sti instance of \ksc.
We recall that each set $S$ of $\mathcal S$ is the union of an $A$-interval with a $B$-interval: $S=S_A \uplus S_B$.
We transform each set $S$ into a $2$-element $(x_{S,A},x_{S,B})$, and each element $u$ of the \ksc instance into a set $T_u$ of the \shs instance. 
We put element $x_{S,A}$ (resp. $x_{S,B}$) into set $T_u$ whenever $u \in S \cap A=I_A$ (resp. $u \in S \cap B=I_B$). 
We call $A'$ (resp. $B'$) the set of all the elements of the form $x_{S,A}$ (resp. $x_{S,B}$).
We shall now specify an order of $A'$ and $B'$ so that the instance is \emph{structured}.
Keep in mind that elements in the \shs instance corresponds to sets in the \ksc instance.
We order the elements of $A'$ accordingly to the following ordering of the sets of the \ksc instance: $\mathcal S_b(1)$, $\mathcal S(1,2)$, $\ldots$, $\mathcal S(1,k)$, $\mathcal S_e(1)$, $\mathcal S_b(2)$, $\mathcal S(2,1)$, $\ldots$, $\mathcal S(2,k)$, $\mathcal S_e(2)$, $\ldots$, $\mathcal S_b(k)$, $\mathcal S(k,1)$, $\ldots$, $\mathcal S(k,k-1)$, $\mathcal S_e(k)$, $\mathcal S(1,2,\vdash)$, $\mathcal S(1,2,\dashv)$, $\mathcal S(1,3,\vdash)$, $\mathcal S(1,3,\dashv)$, $\ldots$, $\mathcal S(k-1,k,\vdash)$, $\mathcal S(k-1,k,\dashv)$. 
We order the elements of $B'$ accordingly to the following ordering of the sets of the \ksc instance: $\mathcal S(1,2,\vdash)$, $\mathcal S(1,2)$, $\mathcal S(2,1)$, $\mathcal S(1,2,\dashv)$, $\mathcal S(1,3,\vdash)$, $\mathcal S(1,3)$, $\mathcal S(3,1)$, $\mathcal S(1,3,\dashv)$, $\ldots$, $\mathcal S(k-1,k,\vdash)$, $\mathcal S(k-1,k)$, $\mathcal S(k,k-1)$, $\mathcal S(k-1,k,\dashv)$, $\mathcal S_b(1)$, $\mathcal S_e(1)$, $\ldots$, $\mathcal S_b(k)$, $\mathcal S_e(k)$. 
Within all those sets of sets, we order by increasing left endpoint (and then, in case of a tie, by increasing right endpoint).
One can now check that with those two orders $\leq_{A'}$ and $\leq_{B'}$, all the sets $T_u$'s are $A'$-interval or $B'$-interval.
Also, one can check that the \textsc{$2$-Track Hitting Set} instance is \emph{structured} by taking as color classes the partite sets $\mathcal S_b(i)$'s, $\mathcal S_e(i)$'s, $\mathcal S(i,j)$'s, $\mathcal S(i,j,\vdash)$'s, and $\mathcal S(i,j,\dashv)$'s.
Now, taking one $2$-element in each color class to hit all the sets $T_u$ corresponds to taking one set in each partite set of $\mathcal S$ to dominate all the elements of the \ksc instance. 
\end{proof}
% }

For the size $|\mathcal I|$ of an instance $\mathcal I$ of \shs, one can take $kt+|\mathcal S_A|+|\mathcal S_B|$.

% \appendixtext{Related results}{

$2$-track (unit) interval graphs are the intersection graphs of (unit) $2$-track intervals, where a (unit) $2$-track interval is the union of two (unit) intervals in two disjoint copies of the real line, called the first track and the second track.
Two $2$-track intervals intersect if they intersect in either the first or the second track.
We observe here that many dominating problems with some geometric flavor can be restated with the terminology of $2$-track (unit) interval graphs. 

In particular, a result almost identical to Corollary~\ref{cor:main} was obtained recently:
\begin{theorem}[\cite{Marx15}]\label{cor:2-track-obj-int}
Given the representation of a $2$-track unit interval graph, the problem of selecting $k$ objects to dominate all the \emph{intervals} is \wone-hard, and not solvable in time $n^{o(k / \log k)}$, unless the ETH fails.
\end{theorem}

We still had to give an \emph{alternative} proof of this result because we will need the additional property that the instance can be further assumed to have the structure depicted in Figure~\ref{fig:permutations}.
This will be crucial for showing the hardness result for \vgag. 
%This corollary is closely related to the following hardness results of Jiang and of Dom et al.

Other results on dominating problems in $2$-track unit interval graphs include: 
\begin{theorem}[\cite{Jiang10}]
Given the representation of a $2$-track unit interval graph, the problem of selecting $k$ objects to dominate all the objects is \wone-hard.
\end{theorem}

\begin{theorem}[\cite{Dom12}]
Given the representation of a $2$-track unit interval graph, the problem of selecting $k$ \emph{intervals} to dominate all the objects is \wone-hard.
\end{theorem}

The result of Dom et al. is formalized differently in their paper \cite{Dom12}, where the problem is defined as stabbing axis-parallel rectangles with axis-parallel lines.
% }

This introductory lemma inspires the \emph{linker} gadgets for both \pgag and \vgag.
\begin{lemma}\label{lem:linking-set-system:pg&vg}
The only minimum hitting sets of the set-system $\mathcal S = \{S_i=\{1,2,\ldots,i,$ $\overline{i+1},\overline{i+2},$ $\ldots,\overline{n}\}$ $|$ $i \in [n]\} \cup \{\overline{S}_i=\{\overline{1},\overline{2},\ldots,\overline{i},i+1,i+2,\ldots,n\}$ $|$ $i \in [n]\}$ are $\{i,\overline{i}\}$, for each $i \in [n]$.
\end{lemma}

% \appendixproof{Lemma~\ref{lem:linking-set-system:pg&vg}}
% {
\begin{proof}
First, for each $i \in [n]$, one may easily observe that $\{i,\overline{i}\}$ is a hitting set of $\mathcal S$.
Now, because of sets $S_n$ and $\overline{S}_n$ one should pick one element $i$ and one element $\overline{j}$ for some $i, j \in [n]$.
If $i < j$, then set $\overline{S}_i$ is not hit, and if $i > j$, then $S_j$ is not hit.
Therefore, $i$ should be equal to $j$.
\end{proof}
% }

\ParaPoint*
% \begin{theorem}
% \pgag parameterized by the number of guards $k$ is \wone-hard, and is not solvable in time $n^{o(k / \log k)}$, under the ETH.
% \end{theorem}



\begin{proof}
We present a reduction from \shs.
Given an instance $\mathcal I=(k \in \mathbb{N},t \in \mathbb{N}, \sigma \in \mathfrak S_k, \sigma_1 \in \mathfrak S_t, \ldots, \sigma_k \in \mathfrak S_t, \mathcal S_A, \mathcal S_B)$, we build a simple polygon $\mathcal P$ with $O(kt+|\mathcal S_A|+|\mathcal S_B|)$ vertices, such that $\mathcal I$ is a YES-instance iff $\mathcal P$ can be guarded by $3k$ points.

We recall that $A$'s order is: $a^1_1, \ldots, a^1_t, \ldots, a^k_1, \ldots, a^k_t$ and $B$'s order is determined by $\sigma$ and the $\sigma_j$'s (see Figure~\ref{fig:permutations}).
The global strategy of the reduction is to \emph{allocate}, for each color class $j \in [k]$, $2t$ special points in the polygon $\alpha^j_1, \ldots, \alpha^j_t$ and $\beta^j_1, \ldots, \beta^j_t$.
Placing a guard in $\alpha^j_i$ (resp.~$\beta^j_i$) shall correspond to picking a $2$-element whose first (resp.~second) component is $a^j_i$ (resp.~$b^j_i$). 
The points $\alpha^j_i$'s and $\beta^j_i$'s ordered by increasing $y$-coordinates will match the order of the $a^j_i$'s along $\leq_A$ and then of the $b^j_i$'s along $\leq_B$.
Then, far in the horizontal direction, we will place pockets to encode each $A$-interval of $\mathcal S_A$, and each $B$-interval of $\mathcal S_B$ (see Figure~\ref{fig:interval-pg&vg}).

The critical issue will be to \emph{link} point $\alpha^j_i$ to point $\beta^j_i$.
Indeed, in the \shs problem, one selects $2$-elements (one per color class), so we should prevent one from placing two guards in $\alpha^j_i$ and $\beta^j_{i'}$ with $i \neq i'$.
The so-called \emph{point linker} gadget will be grounded in Lemma~\ref{lem:linking-set-system:pg&vg}.
Due to a technicality (see Figure~\ref{fig:weak-linker-pg}) we will introduce a \emph{copy} $\overline{\alpha}^j_i$ of each $\alpha^j_i$.
In each part of the gallery encoding a color class $j \in [k]$, the only way of guarding all the pockets with only three guards will be to place them in $\alpha^j_i$, $\overline{\alpha}^j_i$, and $\beta^j_i$ for some $i \in [t]$ (see Figure~\ref{fig:linker-pg}).
Hence, $3k$ guards will be necessary and sufficient to guard the whole $\mathcal P$ iff there is a solution to the instance of \shs.

\begin{figure}
\centering
\resizebox{200pt}{!}
{
\begin{tikzpicture}[scale=1]
\def\pockets{4}
\def\r{7}
\path[name path = p] (\r,1) -- (\r,\pockets+0.5) ;
\foreach \i in {1,...,\pockets}{
\node [vertex,label=right:$z_\i$] (z\i) at (8.5,\i) {} ;
}

\node[point,label=left:$p_1$] (p1) at (-0.3,1.1) {};
\node[point,label=left:$p_2$] (p2) at (0.2,1.6) {};
\node[point,label=left:$p_3$] (p3) at (-0.5,2) {};
\node[point,label=left:$p_4$] (p4) at (0.1,2.5) {};
\node[point,label=left:$p_5$] (p5) at (0,3.2) {};
\node[point,label=left:$p_6$] (p6) at (0.7,3.8) {};

\begin{scope}[thin,opacity=0.5]
\draw[name path global/.expanded=zpa1] (z1) -- (p1) ;
\draw[name path global/.expanded=zpb1] (z1) -- (p3) ;

\draw[name path global/.expanded=zpa2] (z2) -- (p2) ;
\draw[name path global/.expanded=zpb2] (z2) -- (p5) ;

\draw[name path global/.expanded=zpa3] (z3) -- (p4) ;
\draw[name path global/.expanded=zpb3] (z3) -- (p5) ;

\draw[name path global/.expanded=zpa4] (z4) -- (p4) ;
\draw[name path global/.expanded=zpb4] (z4) -- (p6) ;
\end{scope}

\foreach \i in {1,...,\pockets}{
\draw [name intersections={of=p and zpa\i}, very thick] (z\i) -- (intersection-1) coordinate (cza\i) {} ;
\draw [name intersections={of=p and zpb\i}, very thick] (z\i) -- (intersection-1) coordinate (czb\i) {} ; 
}

\foreach \i [count=\j from 1] in {2,...,\pockets}{
\draw[very thick] (cza\i) -- (czb\j) ;
}
\end{tikzpicture}
}
\caption{Interval gadgets encoding $\{p_1,p_2,p_3\}$, $\{p_2,p_3,p_4,p_5\}$, $\{p_3,p_4,p_5\}$, and $\{p_4,p_5,p_6\}$.}
\label{fig:interval-pg&vg}
\end{figure}

We now get into the details of the reduction.
We will introduce several characteristic lengths and compare them; when \emph{$l_1 \ll l_2$} means that $l_1$ should be thought as really small compared to $l_2$, and \emph{$l_1 \approx l_2$} means that $l_1$ and $l_2$ are roughly of the same order.
The motivation is to guide the intuition of the reader without bothering her/him with the details until due time.
At the end of the construction, we will specify those lengths. 

We recall that we want the points $\alpha^j_i$'s and $\beta^j_i$'s ordered by increasing $y$-coordinates, to match the order of the $a^j_i$'s and $b^j_i$'s along $\leq_A$ and $\leq_B$, with first all the elements of $A$ and then all the elements of $B$.
Starting from some $y$-coordinate $y_1$ (which is the one given to point $\alpha^1_1$), the $y$-coordinates of the $\alpha^j_i$'s are regularly spaced out by an offset $y$; that is, the $y$-coordinate of $\alpha^j_i$ will be $y_1+\ord(\alpha^j_i)y=y_1+(i+(j-1)t)y$.
Between the $y$-coordinate of the last element in $A$ (i.e., $a^k_t$ whose $y$-coordinate is $y_1+(kt-1)y$) and the first element in $B$, there is a large offset $L$, such that the $y$-coordinate of $\beta^j_i$ is $y_1+(kt-1)y+L+\ord(\beta^j_i)y$ (for any $j \in [k]$ and $i \in [t]$).

For each color class $j \in [k]$, let $x_j := x_1 + (j-1)D$ for some $x$-coordinate $x_1$ and value $D$, and $y_j := y_1 + (j-1)ty$.
The allocated points $\alpha^j_1, \alpha^j_2, \alpha^j_3, \ldots, \alpha^j_t$ are on a line at coordinates: $(x_j,y_j), (x_j+x,y_j+y), (x_j+2x,y_j+2y), \ldots, (x_j+(t-1)x,y_j+(t-1)y)$, for some value $x$.
We place, to the left of those points, a rectangular pocket $\mathcal P_{j,r}$ of width, say, $y$ and length, say\footnote{the exact width and length of this pocket are not that relevant; the reader may just think of $\mathcal P_{j,r}$ as a thin pocket which forces to place a guard on a thin strip whose uppermost boundary is $\ell(\alpha^j_1,\alpha^j_t)$}, $tx$ such that the uppermost longer side of the rectangular pocket lies on the line $\ell(\alpha^j_1,\alpha^j_t)$ (see Figure~\ref{fig:weak-linker-pg}).
The $y$-coordinates of $\beta^j_1, \beta^j_2, \beta^j_3, \ldots, \beta^j_t$ have already been defined.
We set, for each $i \in [t]$, the $x$-coordinate of $\beta^j_i$ to $x_j+(i-1)x$, so that $\beta^j_i$ and $\alpha^j_i$ share the same $x$-coordinate. 
One can check that it is consistent with the previous paragraph.
We also observe that, by the choice of the $y$-coordinate for the $\beta^j_i$'s, we have both encoded the permutations $\sigma_j$'s and permutation $\sigma$ (see Figure~\ref{fig:overall-pg} or Figure~\ref{fig:weak-linker-pg}).

From hereon, for a vertex $v$ and two points $p$ and $p'$, we informally call \emph{triangular pocket rooted at vertex $v$ and supported by $\ray(v,p)$ and $\ray(v,p')$} a sub-polygon $w, v, w'$ (a triangle) such that $\ray(v,w)$ passes through $p$, $\ray(v,w')$ passes through $p'$, while $w$ and $w'$ are close to $v$ (sufficiently close not to interfere with the rest of the construction).
We say that $r$ is the \emph{root} of the triangular pocket, that we often denote by $\mathcal P(r)$.
We also say that the pocket $\mathcal P(r)$ \emph{points} towards $p$ and $p'$.
At the $x$-coordinate $x_k+(t-1)x+F$, for some large value $F$, we put between $y$-coordinates $y_1$ and $y_k+(kt-1)y$, for each $A$-interval $I_q=[a^j_i,a^{j'}_{i'}] \in \mathcal S_A$ we put one triangular pocket $\mathcal P(z_{A,q})$ rooted at vertex $z_{A,q}$ and supported by $\ray(z_{A,q},\alpha^j_i)$ and $\ray(z_{A,q},\alpha^{j'}_{i'})$.
Intuitively, if $y \ll x \ll D \ll F$, the only $\alpha^{j''}_{i''}$ seeing vertex $z_{A,q}$ should be all the points such that $a^j_i \leq_A a^{j''}_{i''} \leq_A a^{j'}_{i'}$ (see Figure~\ref{fig:overall-pg} and Figure~\ref{fig:interval-pg&vg}).
We place those $|\mathcal S_A|$ pockets along the $y$-axis, and space them out by distance $s$.
To guarantee that we have enough room to place all those pockets, $s \ll y$ shall later hold.
Similarly, we place at the same $x$-coordinate $x_k+(t-1)x+F$ each of the $|\mathcal S_B|$ triangular pockets $\mathcal P(z_{B,q})$ rooted at vertex $z_{B,q}$ and supported by $\ray(z_{B,q},\beta^j_i)$ and $\ray(z_{B,q},\beta^{j'}_{i'})$ for $B$-interval $[b^j_i,b^{j'}_{i'}] \in \mathcal S_B$; and we space out those pockets by distance $s$ along the $y$-axis between $x$-coordinates $y_1+(kt-1)y+L$ and $y_1+2(kt-1)y+L$.
We do not specify an order to the $z_{A,q}$'s (resp.~the $z_{B,q}$'s) along the $y$-axis since we do not need that to prove the reduction correct.
The different values ($s$, $x$, $y$, $D$, $L$, and $F$) introduced so far compare in the following way: $s \ll y \ll x \ll D \ll F$, and $x \ll L \ll F$ (see Figure~\ref{fig:overall-pg}).


Now, we describe how we \emph{link} each point $\alpha^j_i$ to its \asso $\beta^j_i$.
For each $j \in [k]$, let us mentally draw $\ray(\alpha^j_t,\beta^j_1)$ and consider points slightly to the left of this ray at a distance, say, $L'$ from point $\alpha^j_t$.
Let us call $\mathcal R^j_{\text{left}}$ that informal region of points.
Any point in $\mathcal R^j_{\text{left}}$ sees, from right to left, in this order $\alpha^j_1$, $\alpha^j_2$ up to $\alpha^j_t$, and then, $\beta^j_1$, $\beta^j_2$ up to $\beta^j_t$.
This observation relies on the fact that $y \ll x \ll L$.
So, from the distance, the points $\beta^j_1, \ldots, \beta^j_t$ look almost \emph{flat}.
It makes the following construction possible.
In $\mathcal R^j_{\text{left}}$, for each $i \in [t-1]$, we place a triangular pocket $\mathcal P(c^j_i)$ rooted at vertex $c^j_i$ and supported by $\ray(c^j_i,\alpha^j_{i+1})$ and $\ray(c^j_i,\beta^j_i)$. 
We place also a triangular pocket $\mathcal P(c^j_t)$ rooted at $c^j_t$ supported by $\ray(c^j_i,\beta^j_1)$ and $\ray(c^j_i,\beta^j_t)$.
We place vertices $c^j_i$ and $c^j_{i+1}$ at the same $y$-coordinate and spaced out by distance $x$ along the $x$-axis (see Figure~\ref{fig:weak-linker-pg}).
Similarly, let us informally refer to the region slightly to the right of $\ray(\alpha^j_1,\beta^j_t)$ at a distance $L'$ from point $\alpha^j_1$, as $\mathcal R^j_{\text{right}}$.
Any point $\mathcal R^j_{\text{right}}$ sees, from right to left, in this order $\beta^j_1$, $\beta^j_2$ up to $\beta^j_t$, and then, $\alpha^j_1$, $\alpha^j_2$ up to $\alpha^j_t$.
Therefore, one can place in $\mathcal R^j_{\text{left}}$, for each $i \in [t-1]$, a triangular pocket $\mathcal P(d^j_i)$ rooted at $d^j_i$ supported by $\ray(d^j_i,\beta^j_{i+1})$ and $\ray(c^j_i,\alpha^j_i)$.
We place also a triangular pocket $\mathcal P(d^j_t)$ rooted at $d^j_t$ supported by $\ray(d^j_i,\alpha^j_1)$ and $\ray(c^j_i,\alpha^j_t)$.
Again, those $t$ pockets can be put at the same $y$-coordinate and spaced out horizontally by $x$ (see Figure~\ref{fig:weak-linker-pg}).
We denote by $\mathcal P_{j,\alpha,\beta}$ the set of pockets $\{\mathcal P(c^j_1), \ldots, \mathcal P(c^j_t), \mathcal P(d^j_1), \ldots, \mathcal P(d^j_t)\}$ and informally call it the \emph{weak point linker} (or simply, \emph{weak linker}) of $\alpha^j_1, \ldots, \alpha^j_t$ and $\beta^j_1, \ldots, \beta^j_t$.
We may call the pockets of $\mathcal R^j_{\text{left}}$ (resp. $\mathcal R^j_{\text{right}}$) \emph{left} pockets (resp. \emph{right} pockets).

\begin{figure}
\centering
\resizebox{250pt}{!}
{
\begin{tikzpicture}[scale=0.35]
\foreach \i in {1,...,6}{
\node[point,label=below:$\alpha_\i$] (a\i) at (\i,0.1 * \i) {} ;
}

\node[point,label=above:$\beta_1$] (b1) at (1,8.4) {} ;
\node[point,label=above:$\beta_2$] (b2) at (2,8.7) {} ;
\node[point,label=above:$\beta_3$] (b3) at (3,8.1) {} ;
\node[point,label=above:$\beta_4$] (b4) at (4,8.2) {} ;
\node[point,label=above:$\beta_5$] (b5) at (5,8.6) {} ;
\node[point,label=above:$\beta_6$] (b6) at (6,8.3) {} ;

\foreach \i in {1,...,6}{
\coordinate (cb\i) at (b\i) ;
}

% points inside the pockets: c_i and d_i
\path [name path = p] (-16,21.5) -- (23,21.5) ;
\foreach \i in {1,...,6}{
\node [vertex,label=above:$d_\i$] (c\i) at (17+\i,23) {} ;
\draw [name path global/.expanded=e\i,very thin] (c\i) -- (a\i) ;
\node [vertex,label=above:$c_\i$] (d\i) at (-17+\i,23) {} ;
\draw [name path global/.expanded=g\i,very thin] (d\i) -- ($(b\i)!-0.7cm!(d\i)$) coordinate (q\i) ;
}

\foreach \i [count=\j from 2] in {1,...,5}{
\draw[name path global/.expanded=f\i,very thin] (c\i) -- ($(b\j)!-0.7cm!(c\i)$) coordinate (p\i) ;       
}

\draw[name path = f6, very thin] (c6) -- (a1) ;  

%\node[fill=(p2) (q2) (b2)] (y2) {} ;


\draw[name path = h6, very thin] (d6) -- ($(b1)!-0.7cm!(d6)$) coordinate (p6) ;

\foreach \i [count=\j from 2] in {1,...,5}{
\draw[name path global/.expanded=h\i, very thin] (d\i) -- (a\j) ;       
}

\foreach \i in {1,...,6}{
\draw [name intersections={of=p and e\i}, very thick] (c\i) -- (intersection-1) coordinate (s\i) {} ; 
\draw [name intersections={of=p and f\i}, very thick] (c\i) -- (intersection-1) coordinate (t\i) {} ; 
\draw [name intersections={of=p and g\i}, very thick] (d\i) -- (intersection-1) coordinate (u\i) {} ; 
\draw [name intersections={of=p and h\i}, very thick] (d\i) -- (intersection-1) coordinate (v\i) {} ; 
}

\foreach \i [count=\j from 2] in {1,...,5}{
\draw[very thick] (s\i) -- (t\j) ; 
\draw[very thick] (u\i) -- (v\j) ;       
}

\draw[very thick] (u6) -- (t1) ;

\begin{scope}[opacity=0.5]
\foreach \i [count = \j from 2] in {1,...,5}{
\fill (cb\j) -- (p\i) -- (q\j) ;
}
\fill (cb1) -- (p6) -- (q1) ;
\end{scope}

\begin{scope}[xshift=-9cm,yshift=-0.9cm]
\draw[very thick] (6,0.5) -- (1,0) -- (1,0.2) -- (6,0.7)  ;
\end{scope}

\end{tikzpicture}
}
\caption{Weak point linker gadget.}
\label{fig:weak-linker-pg}
\end{figure}

As we will show later, if one wants to guard with only two points all the pockets of $\mathcal P_{j,\alpha,\beta} = \{\mathcal P(c^j_1), \ldots, \mathcal P(c^j_t), \mathcal P(d^j_1), \ldots, \mathcal P(d^j_t)\}$ and one first decides to put a guard on point $\alpha^j_i$ (for some $i \in [t]$), then one is not forced to put the other guard on point $\beta^j_i$ but only on an area whose uppermost point is $\beta^j_i$ (see the shaded areas below the $b^j_i$'s in Figure~\ref{fig:weak-linker-pg}).
Now, if $\beta^j_1, \ldots, \beta^j_t$ would all lie on a same line $\ell$, we could shrink the shaded area of each $\beta^j_i$ (Figure~\ref{fig:weak-linker-pg}) down to the single point $\beta^j_i$ by adding a thin rectangular pocket on $\ell$ (similarly to what we have for $\alpha^j_1, \ldots, \alpha^j_t$).
Naturally we need $\beta^j_1, \ldots, \beta^j_t$ \emph{not} to be on the same line to be able to encode $\sigma_j$.
The remedy we suggest is the following.
For each $j \in [k]$, we allocate $t$ points $\overline{\alpha}^j_1, \overline{\alpha}^j_2, \ldots, \overline{\alpha}^j_t$ on a horizontal line, spaced out by distance $x$, say, $\approx \frac{D}{2}$ to the right and $\approx L$ to the up of $\beta^j_t$.
We put a thin horizontal rectangular pocket $\mathcal P_{j,\overline{r}}$ of the same dimension as $\mathcal P_{j,r}$ such that the lowermost longer side of $\mathcal P_{j,\overline{r}}$ is on the line $\ell(\overline{\alpha}^j_1,\overline{\alpha}^j_t)$.
We add the $2t$ pockets corresponding to a weak linker $\mathcal P_{j,\alpha,\overline{\alpha}}$ between $\alpha^j_1, \ldots, \alpha^j_t$ and $\overline{\alpha}^j_1, \ldots, \overline{\alpha}^j_t$ as well as the $2t$ pockets of a weak linker $\mathcal P_{j,\overline{\alpha},\beta}$ between $\overline{\alpha}^j_1, \ldots, \overline{\alpha}^j_t$ and $\beta^j_1, \ldots, \beta^j_t$ as pictured in Figure~\ref{fig:linker-pg}.
We denote by $\mathcal P_j$ the union $\mathcal P_{j,r} \cup \mathcal P_{j,\overline{r}} \cup \mathcal P_{j,\alpha,\beta} \cup \mathcal P_{j,\alpha,\overline{\alpha}} \cup \mathcal P_{j,\overline{\alpha},\beta}$ of all the pockets involved in the encoding of color class $j$.
Now, say, one wants to guard all the pockets of $\mathcal P_j$ with only three points, and chooses to put a guard on $\alpha^j_i$ (for some $i \in [t]$).
Because of the pockets of $\mathcal P_{j,\alpha,\overline{\alpha}} \cup P_{j,\overline{r}}$, one is forced to place a second guard precisely on $\overline{\alpha}^j_i$.
Now, because of the weak linker $\mathcal P_{j,\alpha,\beta}$ the third guard should be on a region whose uppermost point is $\beta^j_i$, while, because of $\mathcal P_{j,\overline{\alpha},\beta}$ the third guard should be on a region whose lowermost point is $\beta^j_i$.
The conclusion is that the third guard should be put precisely on $\beta^j_i$. 
This \emph{triangle} of weak linkers is called the \emph{linker} of color class $j$. 
The $k$ linkers are placed accordingly to Figure~\ref{fig:overall-pg}.
This ends the construction.

\begin{figure}
\centering
\resizebox{250pt}{!}
{
\begin{tikzpicture}[scale=0.15]
\foreach \i in {1,...,6}{
\node[spoint] (a\i) at (\i,0.1 * \i-12) {} ;
}

\begin{scope}[xshift=35cm,yshift=30cm]
\foreach \i in {1,...,6}{
\node[spoint] (zb\i) at (\i-6,-3) {} ;
\coordinate (zc\i) at (11+1.5 * \i,10) {} ;
\coordinate (zd\i) at (-3+\i,10) {} ;
}
\end{scope}

\foreach \i in {1,...,6}{
\coordinate (yc\i) at (-35,-3 - 0.7 * \i) {} ;
\coordinate (yd\i) at (-35,10 -0.7 * \i) {} ;
}

\path [name path = zp] (0,38) -- (70,38) ;
\path [name path = yp]  (-33,-10) -- (-33,20) ;


\begin{scope}[yshift=8cm]
\node[spoint] (b1) at (1,8.4) {} ;
\node[spoint] (b2) at (2,8.7) {} ;
\node[spoint] (b3) at (3,8.1) {} ;
\node[spoint] (b4) at (4,8.2) {} ;
\node[spoint] (b5) at (5,8.6) {} ;
\node[spoint] (b6) at (6,8.3) {} ;
\end{scope}


%\draw (zb1) -- (yc1) ;
%\draw (zb6) -- (yd6) ;

% Linker a_i <-> b_i
\path [name path = p] (-16,28.5) -- (23,28.5) ;

\begin{scope}[yshift=7cm]
\foreach \i in {1,...,6}{
\coordinate (c\i) at (17+\i,23) {} ;
\draw [name path global/.expanded=e\i,green,very thin] (c\i) -- (a\i) ;
\coordinate (d\i) at (-17+\i,23) {} ;
\draw [name path global/.expanded=g\i,green,very thin] (d\i) -- ($(b\i)!-0.7cm!(d\i)$) coordinate (q\i) ;
}
\end{scope}

\foreach \i [count=\j from 2] in {1,...,5}{
\draw[name path global/.expanded=f\i,green,very thin] (c\i) -- ($(b\j)!-0.7cm!(c\i)$) coordinate (p\i) ;       
}

\draw[name path = f6, green,very thin] (c6) -- (a1) ;  

\draw[name path = h6, green,very thin] (d6) -- ($(b1)!-0.7cm!(d6)$) coordinate (p6) ;

\foreach \i [count=\j from 2] in {1,...,5}{
\draw[name path global/.expanded=h\i, green,very thin] (d\i) -- (a\j) ;       
}

\foreach \i in {1,...,6}{
\draw [name intersections={of=p and e\i}, very thick] (c\i) -- (intersection-1) coordinate (s\i) {} ; 
\draw [name intersections={of=p and f\i}, very thick] (c\i) -- (intersection-1) coordinate (t\i) {} ; 
\draw [name intersections={of=p and g\i}, very thick] (d\i) -- (intersection-1) coordinate (u\i) {} ; 
\draw [name intersections={of=p and h\i}, very thick] (d\i) -- (intersection-1) coordinate (v\i) {} ; 
}

\foreach \i [count=\j from 2] in {1,...,5}{
\draw[very thick] (s\i) -- (t\j) ; 
\draw[very thick] (u\i) -- (v\j) ;       
}

\draw[very thick] (u6) -- (t1) ;

% Linker a_i's <-> mirror of a_i's

\foreach \i in {1,...,6}{
\draw [name path global/.expanded=ze\i,blue,very thin] (zc\i) -- (a\i) ;
\draw [name path global/.expanded=zg\i,blue,very thin] (zd\i) -- (zb\i) coordinate (zq\i) ;
}

\foreach \i [count=\j from 2] in {1,...,5}{
\draw[name path global/.expanded=zf\i,blue,very thin] (zc\i) -- (zb\j) coordinate (zp\i) ;       
}

\draw[name path = zf6, blue,very thin] (zc6) -- (a1) ;  

\draw[name path = zh6, blue,very thin] (zd6) -- (zb1) coordinate (zp6) ;

\foreach \i [count=\j from 2] in {1,...,5}{
\draw[name path global/.expanded=zh\i, blue,very thin] (zd\i) -- (a\j) ;       
}

\foreach \i in {1,...,6}{
\draw [name intersections={of=zp and ze\i}, very thick] (zc\i) -- (intersection-1) coordinate (zs\i) {} ; 
\draw [name intersections={of=zp and zf\i}, very thick] (zc\i) -- (intersection-1) coordinate (zt\i) {} ; 
\draw [name intersections={of=zp and zg\i}, very thick] (zd\i) -- (intersection-1) coordinate (zu\i) {} ; 
\draw [name intersections={of=zp and zh\i}, very thick] (zd\i) -- (intersection-1) coordinate (zv\i) {} ; 
}

\foreach \i [count=\j from 2] in {1,...,5}{
\draw[very thick] (zs\i) -- (zt\j) ; 
\draw[very thick] (zu\i) -- (zv\j) ;       
}

\draw[very thick] (zu6) -- (zt1) ;

%\begin{scope}[xshift=20cm,yshift=31.8cm]
%\draw[very thick] (zv1) -- (6,-0.4) -- (1,0.1) -- (1,-0.3) -- (6,-0.8) -- (s6) ;
%\end{scope}
\draw[very thick] (zv1) -- (s6) ;

% Linker mirror of a_i's <-> b_i's

\foreach \i in {1,...,6}{
\draw [name path global/.expanded=ye\i,red, very thin] (yc\i) -- (zb\i) ;
\draw [name path global/.expanded=yg\i,red, very thin] (yd\i) -- ($(b\i)!-0.7cm!(yd\i)$) coordinate (yq\i) ;
}

\foreach \i [count=\j from 2] in {1,...,5}{
\draw[name path global/.expanded=yf\i,red, very thin] (yc\i) -- ($(b\j)!-0.7cm!(yc\i)$) coordinate (yp\i) ;       
}

\draw[name path = yf6, red, very thin] (yc6) -- (zb1) ;  

\draw[name path = yh6, red, very thin] (yd6) -- ($(b1)!-0.7cm!(yd6)$) coordinate (yp6) ;

\foreach \i [count=\j from 2] in {1,...,5}{
\draw[name path global/.expanded=yh\i, red, very thin] (yd\i) -- (zb\j) ;       
}

\foreach \i in {1,...,6}{
\draw [name intersections={of=yp and ye\i}, very thick] (yc\i) -- (intersection-1) coordinate (ys\i) {} ; 
\draw [name intersections={of=yp and yf\i}, very thick] (yc\i) -- (intersection-1) coordinate (yt\i) {} ; 
\draw [name intersections={of=yp and yg\i}, very thick] (yd\i) -- (intersection-1) coordinate (yu\i) {} ; 
\draw [name intersections={of=yp and yh\i}, very thick] (yd\i) -- (intersection-1) coordinate (yv\i) {} ; 
}

\foreach \i [count=\j from 2] in {1,...,5}{
\draw[very thick] (ys\i) -- (yt\j) ; 
\draw[very thick] (yu\i) -- (yv\j) ;       
}

\draw[very thick] (yu6) -- (yt1) ;
\begin{scope}[yshift=2cm]
\draw[very thick] (yv1) -- (-20,25) -- (-26,25) -- (-26,25.5) -- (-20,25.5) -- (v1) ;
\end{scope}

\begin{scope}[xshift=-20cm,yshift=-13.5cm]
\draw[very thick] (6,0.4) -- (1,-0.1) -- (1,0.3) -- (6,0.8) -- (ys6) ;
\end{scope}
\end{tikzpicture}
}
\caption{Point linker gadget: a triangle of (three) weak point linkers.}
\label{fig:linker-pg}
\end{figure}

\begin{figure}
\includegraphics{PointGuardBigPictureSmall2}
\caption{The overall picture of the reduction with $k=3$.}
\label{fig:overall-pg}
\end{figure}

% \appendixtext{Length specification}{
%begin clearly appendixable part
%We now explicit $s, x, y, D, L, L', F$ for our assumptions to be fulfilled.
We can specify the coordinates of positions of all the vertices by fractions of integers. 
These integers are polynomially bounded in $n$. If we want to get integer coordinates, we can transform the rational coordinates to integer coordinates by multiplying all of them with the least common multiple of all the denominators, which is not polynomially bounded anymore. The length of the integers in binary is still polynomially bounded.

In this extended abstract, we give only $s, y$ and $F$ explicitly. 
We can safely set $s$ to one, as it is the smallest length, we specified.
We will put $|\mathcal{S}_a|$ pockets on track $1$ and $|\mathcal{S}_b|$ pockets on track $2$. 
It is sufficient to have an opening space of one between them. Thus, the space on the right side of $\mathcal{P}$,
for all pockets of track $1$ is bounded by $2\cdot |\mathcal{S}_a|$. Thus setting $y$ to $|\mathcal{S}_a| + |\mathcal{S}_b|$ secures us that we have plenty of space to place all the pockets.
We specify $F = (|\mathcal{S}_a|+|\mathcal{S}_b|) D k = y\cdot D \cdot k$. We have to show that this is large enough to guarantee that the pockets on track $1$  distinguish the picked points only by the $y$-coordinate. Let $p$ and $q$ be two points among the $\alpha_{i}^j$. Their vertical distance is upper bounded by $D k$ and their horizontal distance is lower bounded by $y$. Thus the slope of $\ell = \ell(p,q)$ is at least $\tfrac{y}{Dk}$. At the right side of $\mathcal{P}$ the line $\ell$ will be at least $F \tfrac{y}{Dk}$ above the pockets of track $1$. 
Note $F \tfrac{y}{Dk} = y D k \cdot \tfrac{y}{Dk}  > y^2 > |\mathcal{S}_a|^2 > 2\cdot |\mathcal{S}_a|$.  The same argument shows that $F$ is sufficiently large for track $2$. 

The remaining lengths $x, L, L'$, and $D$ can be specified in a similar fashion.
For the construction of the pockets, let $s\in\mathcal{S}_a$ be an $A$-interval with endpoints $a$ and $b$, represented by some points $p$ and $q$ and assume the opening vertices $v$ and $w$ of the triangular pocket are already specified. Then the two lines $\ell(p,v)$ and $\ell(q,w)$ will meet at some point $x$ to the right of $v$ and $w$. By the same arguments given in Lemma~\ref{lem:distances} $x$ has rational coordinates and the integers to represent them can be expressed by the coordinates of $p, q, v,$ and $w$.
This way, all the pockets can be explicitly constructed using rational coordinates as claimed above.
%end clearly appendixable part
% }

\begin{lemma}\label{positive:pg}
$\forall j \in [k]$, $\forall i \in [t]$, the three \asso points $\alpha^j_i$, $\overline{\alpha}^j_i$, $\beta^j_i$ guard entirely $\mathcal P_j$.
\end{lemma}

%\appendixproof{Lemma~\ref{main:pg}}
{
\begin{proof}
%For any $i \in [t]$, three guards placed on \asso points $\alpha^j_i$, $\overline{\alpha}^j_i$, $\beta^j_i$ jointly see all the pockets of $\mathcal P_j$ (that is, we recall, all the pockets of the linker gadget for color class $j$).
The rectangular pockets $\mathcal P_{j,r}$ and $\mathcal P_{j,\overline{r}}$ are entirely seen by respectively $\alpha^j_i$ and  $\overline{\alpha}^j_i$.
The pockets $\mathcal P(c^j_1), \mathcal P(c^j_2), \ldots \mathcal P(c^j_{i-1})$ and $\mathcal P(d^j_i), \mathcal P(d^j_{i+1}), \ldots \mathcal P(d^j_t)$ are all entirely seen by $\alpha^j_i$, while the pockets $\mathcal P(c^j_i), \mathcal P(c^j_{i+1}), \ldots \mathcal P(c^j_t)$ and $\mathcal P(d^j_1), \mathcal P(d^j_2), \ldots \mathcal P(d^j_{i-1})$ are all entirely seen by $\beta^j_i$.
This means that $\alpha^j_i$ and $\beta^j_i$ jointly see all the pockets of $\mathcal P_{j,\alpha,\beta}$.
Similarly, $\alpha^j_i$ and $\overline{\alpha}^j_i$ jointly see all the pockets of $\mathcal P_{j,\alpha,\overline{\alpha}}$, and $\overline{\alpha}^j_i$ and $\beta^j_i$ jointly see all the pockets of $\mathcal P_{j,\overline{\alpha},\beta}$.
Therefore, $\alpha^j_i$, $\overline{\alpha}^j_i$, $\beta^j_i$ jointly see all the pockets of $\mathcal P_j$.
\end{proof}
}

Let us prove the correctness of the reduction.
Assume that $\mathcal I$ is a YES-instance and let $\{(a^1_{s_1},b^1_{s_1}), \ldots, (a^k_{s_k},b^k_{s_k})\}$ be a solution.
We claim that $G=\{\alpha^1_{s_1},\overline{\alpha}^1_{s_1},\beta^1_{s_1}, \ldots, \alpha^k_{s_k},\overline{\alpha}^k_{s_k},\beta^k_{s_k}\}$ guard the whole polygon $\mathcal P$.
By Lemma~\ref{positive:pg}, $\forall j \in [k]$, $\mathcal P_j$ is guarded.
For each $A$-interval (resp.~$B$-interval) in $\mathcal S_A$ (resp.~$\mathcal S_B$) there is at least one $2$-element $(a^j_{s_j},b^j_{s_j})$ such that $a^j_{s_j} \in \mathcal S_A$ (resp. $b^j_{s_j} \in \mathcal S_B$).
Thus, the corresponding pocket is guarded by $\alpha^j_{s_j}$ (resp.~$\beta^j_{s_j}$).
The rest of the polygon $\mathcal P$ (which is not part of pockets) is guarded by, for instance, $\{\overline{\alpha}^1_{s_1}, \ldots, \overline{\alpha}^k_{s_k}\}$.
So, $G$ is indeed a solution and it contains $3k$ points.

Assume now that there is no solution to the instance $\mathcal I$ of \shs.
We show that there is no set of $3k$ points guarding $\mathcal P$.
We observe that no point of $\mathcal P$ sees inside two triangular pockets one being in $\mathcal P_{j,\alpha,\gamma}$ and the other in $\mathcal P_{j',\alpha,\gamma'}$ with $j \neq j'$ and $\gamma, \gamma' \in \{\beta,\overline{\alpha}\}$.
Further, $V(r(\mathcal P_{j,\alpha,\beta} \cup \mathcal P_{j,\alpha,\overline{\alpha}})) \cap V(r(\mathcal P_{j',\alpha,\beta} \cup \mathcal P_{j',\alpha,\overline{\alpha}})) = \emptyset$ when $j \neq j'$, where $r$ maps a set of triangular pockets to the set of their root.
Also, for each $j \in [k]$, seeing entirely $\mathcal P_{j,\alpha,\beta}$ and $\mathcal P_{j,\alpha,\overline{\alpha}}$ requires at least $3$ points.
This means that for each $j \in [k]$, one should place three guards in $V(r(\mathcal P_{j,\alpha,\beta} \cup \mathcal P_{j,\alpha,\overline{\alpha}}))$.
Furthermore, one can observe among those three points one should guard a triangular pocket $\mathcal P_{j',r}$ and another should guard $\mathcal P_{j'',\overline{r}}$.
Let us try to guard entirely $\mathcal P_1$ and two rectangular pockets $\mathcal P_{j',r}$ and $\mathcal P_{j'',\overline{r}}$, with only three guards.
Let call $\ell_1$ (resp. $\ell'_1$) the line corresponding to the extension of the uppermost (resp. lowermost) longer side of $\mathcal P_{1,r}$ (resp. $\mathcal P_{1,\overline{r}}$).
The only points of $\mathcal P$ that can see a rectangular pocket $\mathcal P_{j',r}$ and at least $t$ pockets of $\mathcal P_{1,\alpha,\overline{\alpha}}$ are on $\ell_1$: more specifically, they are the points $\alpha^1_1, \ldots, \alpha^1_t$.
 The only points that can see a rectangular pocket $\mathcal P_{j'',\overline{r}}$ and at least $t$ pockets of $\mathcal P_{1,\alpha,\overline{\alpha}}$ are on $\ell'_1$: they are the points $\overline{\alpha}^1_1, \ldots, \overline{\alpha}^1_t$.
As $\mathcal P_{1,\alpha,\overline{\alpha}}$ has $2t$ pockets, one has to take a point $\alpha^1_i$ and $\overline{\alpha}^1_{i'}$.
By the same argument argument as in Lemma~\ref{lem:linking-set-system:pg&vg}, $i$ should be equal to $i'$ (otherwise, $i<i'$ and the left pocket pointing towards $\overline{\alpha}^1_{i'-1}$ and $\alpha^1_{i'}$ is not seen, or $i>i'$ and the right pocket pointing towards $\alpha^1_{i+1}$ and $\overline{\alpha}^1_i$ is not seen).
We now denote by $s_1$ this shared value.
Now, to see left pocket $\mathcal P(c^1_{s_1})$ and right pocket $\mathcal P(d^1_{s_1-1})$ (which are still to be seen), the third guard should be to the left of $\ell(c^1_{s_1},\beta^1_{s_1})$ and to the right of $\ell(d^1_{s_1-1},\beta^1_{s_1})$ (see shaded area of Figure~\ref{fig:weak-linker-pg}).
That is, the third guard should be on a region in which $\beta^1_{s_1}$ is the uppermost point.
The same argument with the pockets of $\mathcal P_{1,\overline{\alpha},\beta}$ implies that the third guard should also be on a region in which $\beta^1_{s_1}$ is the lowermost point.
Thus, the position of the third guard has to be point $\beta^1_{s_1}$.
Therefore, one should put guards on points $\alpha^1_{s_1}$, $\overline{\alpha}^1_{s_1}$, and $\beta^1_{s_1}$, for some $\alpha_1 \in [t]$.

As none of those three points see any pocket $\mathcal P_{j,\overline{\alpha},\beta}$ with $j>1$ (we already mentioned that no pocket of $\mathcal P_{j,\alpha,\beta}$ and $\mathcal P_{j,\alpha,\overline{\alpha}}$ with $j>1$ can be seen by those points), we can repeat the argument for the second color class; and so forth up to color class $k$. 
%By Lemma~\ref{main:pg}, $\forall j \in [k]$, to guard $\mathcal P_j$ with $3$ points one should place guards at $\alpha^j_{s_j},\overline{\alpha}^j_{s_j},\beta^j_{s_j}$ for some $s_j \in [t]$.
%Also, to guard $\mathcal P_j$ at all one should take ... \todo{argument that the color classes do not interact}
Thus, a potential solution with $3k$ guards should be of the form $\{\alpha^1_{s_1},\overline{\alpha}^1_{s_1},\beta^1_{s_1}, \ldots, \alpha^k_{s_k},\overline{\alpha}^k_{s_k},\beta^k_{s_k}\}$.
As there is no solution to $\mathcal I$, there should be a set in $\mathcal S_A \cup \mathcal S_B$ that is not hit by $\{(a^1_{s_1},b^1_{s_1}), \ldots, (a^k_{s_k},b^k_{s_k})\}$.
By construction, the pocket associated to this set is not entirely seen.
\end{proof}

% \begin{theorem}
% \vgag is \wone-hard, and is not solvable in time $n^{o(k / \log k)}$, under the ETH.
% \end{theorem}

 \ParaVertex*

\begin{proof}
Again, we reduce from \shs.
From an instance $\mathcal I=(k \in \mathbb{N},t \in \mathbb{N}, \sigma \in \mathfrak S_k, \sigma_1 \in \mathfrak S_t, \ldots, \sigma_k \in \mathfrak S_t, \mathcal S_A, \mathcal S_B)$, we build a simple polygon $\mathcal P$ with $O(kt+|\mathcal S_A|+|\mathcal S_B|)$ vertices, such that $\mathcal I$ is a YES-instance iff $\mathcal P$ can be guarded by $3k$ vertices.

For each $j \in [k]$, permutation $\sigma_j$ will be encoded by a sub-polygon $\mathcal P_j$ that we call \emph{vertex linker}, or simply \emph{linker} (see Figure~\ref{fig:linker-vg}).
We regularly set $t$ consecutive vertices $\alpha^j_1, \alpha^j_2, \ldots, \alpha^j_t$ in this order, along the $x$-axis.
Opposite to this \emph{segment}, we place $t$ vertices $\beta^j_{\sigma_j(1)}, \beta^j_{\sigma_j(2)}, \ldots, \beta^j_{\sigma_j(t)}$ in this order, along the $x$-axis, too.
The $\beta^j_{\sigma_j(1)}, \ldots, \beta^j_{\sigma_j(t)}$, contrary to $\alpha^j_1, \ldots, \alpha^j_t$, are \emph{not} consecutive.
We will later add some reflex vertices between them.
At mid-distance between $\alpha^j_1$ and $\beta^j_{\sigma_j(1)}$, to the left, we put a reflex vertex $r^j_{\downarrow}$.
\emph{Behind} this reflex vertex, we place a vertical \emph{wall} $d^je^j$ ($r^j_{\downarrow}$, $d^j$, and $e^j$ are three consecutive vertices of $\mathcal P$), so that $\ray(\alpha^j_1,r^j_{\downarrow})$ and $\ray(\alpha^j_t,r^j_{\downarrow})$ both intersect $\seg(d^j,e^j)$. 
That implies that for each $i \in [t]$, $\ray(\alpha^j_i,r^j_{\downarrow})$ intersects $\seg(d^j,e^j)$. 
We denote by point $p^j_i$ this intersection. 
We observe that the greater $i$, the closer to $d^j$. 
Similarly, at mid-distance between $\alpha^j_t$ and $\beta^j_{\sigma_j(t)}$, to the right, we put a reflex vertex $r^j_{\uparrow}$ and place a vertical wall $x^jy^j$ ($r^j_{\uparrow}$, $x^j$, and $y^j$ are consecutive), so that $\ray(\alpha^j_1,r^j_{\uparrow})$ and $\ray(\alpha^j_t,r^j_{\uparrow})$ both intersect $\seg(x^j,y^j)$. 
For each $i \in [t]$, we denote by $q^j_i$ the intersection between $\ray(\alpha^j_i,r^j_{\uparrow})$ and $\seg(x^j,y^j)$.
We observe that the smaller $i$, the closer to $x^j$. 

For each $i \in [t]$, we put around $\beta^j_i$ two reflex vertices, one in $\ray(\beta^j_i,p^j_i)$ and one in $\ray(\beta^j_i,q^j_i)$.
In Figure~\ref{fig:linker-vg}, we merged some reflex vertices but the essential part is that $V(\beta^j_i) \cap \segm(d^j,e^j)=\segm(d^j,p^j_i)$ and $V(\beta^j_i) \cap \segm(x^j,y^j)=\segm(x^j,q^j_i)$.
Finally, we add a triangular pocket rooted at $g^j$ and supported by $\ray(g^j,\alpha^j_1)$ and $\ray(g^j,\alpha^j_t)$, as well as a triangular pocket rooted at $b^j$ and supported by $\ray(g^j,\beta^j_{\sigma_j(1)})$ and $\ray(g^j,\beta^j_{\sigma_j(t)})$.
This ends the description of the vertex linker (see Figure~\ref{fig:linker-vg}).

\begin{figure}[h]
\centering
\resizebox{250pt}{!}
{
\begin{tikzpicture}[scale=1,extended line/.style={shorten >=-#1,shorten <=-#1}, extended line/.default=1cm]

% Vertices meant for track 1

\foreach \i in {1,...,6}{
\node (t\i) at (\i - 1,-0.4) {$\alpha_\i$} ;
\node[vertex] (v\i) at (\i - 1,0) {} ;
}
\draw[very thick] (v1) -- (v6) ;

% Vertices meant for track 2 (arbitrary permutation)

\node (tp1) at (0, 6.4) {$\beta_4$} ;
\node (tp2) at (1, 6.4) {$\beta_2$} ;
\node (tp3) at (2, 6.4) {$\beta_5$} ;
\node (tp4) at (3, 6.4) {$\beta_3$} ;
\node (tp5) at (4, 6.4) {$\beta_6$} ;
\node (tp6) at (5, 6.4) {$\beta_1$} ;

\foreach \i in {1,...,6}{
\node[vertex] (vp\i) at (\i-1, 6) {} ;
}

%pockets A and B

\node[vertex, label=south:$r_{\downarrow}$] (p1) at (-2,3) {} ;
\node[vertex, label=below:$d$] (p2) at (-3,3) {} ;
\node[vertex, label=left:$e$] (p3) at (-3,5) {} ;
\node[vertex, label=north west:$f$] (p4) at (-2,5) {} ;
\node[vertex, label=below:$a$] (u1) at (-0.66,1) {} ;
\node[vertex, label=left:$c$] (u2) at (-1.33,2) {} ;
\draw[very thick] (v1) -- (u1) ;
\draw[very thick] (u2) -- (p1) -- (p2) -- (p3) -- (p4) ;
\path [name path=pocketA] (p2) -- (p3) ;

\node[vertex, label=below:$r_{\uparrow}$] (q1) at (7,3) {} ;
\node[vertex, label=below:$x$] (q2) at (8,3) {} ;
\node[vertex, label=above:$y$] (q3) at (8,5) {} ;
\draw[very thick] (q1) -- (q2) -- (q3) ;
\path [name path=pocketB] (q2) -- (q3) ;

\foreach \i in {1,...,6}{
\path [name path global/.expanded=visa\i] (v\i) -- ($(p1)!-1.8cm!(v\i)$);
\draw [name intersections={of=pocketA and visa\i}, very thin] (v\i) -- (intersection-1) coordinate (e\i) ;
\path [name path global/.expanded=visb\i] (v\i) -- ($(q1)!-1.8cm!(v\i)$);
\draw [name intersections={of=pocketB and visb\i}, very thin] (v\i) -- (intersection-1) coordinate (f\i) ;
}

\draw[very thin] (e1) -- (vp6) -- (f1) ;
\draw[very thin] (e2) -- (vp2) -- (f2) ;
\draw[very thin] (e3) -- (vp4) -- (f3) ;
\draw[very thin] (e4) -- (vp1) -- (f4) ;
\draw[very thin] (e5) -- (vp3) -- (f5) ;
\draw[very thin] (e6) -- (vp5) -- (f6) ;

\path [name path global/.expanded=r1] (e2) -- (vp2) ;
\path [name path global/.expanded=r2] (e5) -- (vp3) ;
\path [name path global/.expanded=r3] (e3) -- (vp4) ;
\path [name path global/.expanded=r4] (e6) -- (vp5) ;
\path [name path global/.expanded=r5] (e1) -- (vp6) ;

\path [name path global/.expanded=s1] (f4) -- (vp1) ;
\path [name path global/.expanded=s2] (f2) -- (vp2) ;
\path [name path global/.expanded=s3] (f5) -- (vp3) ;
\path [name path global/.expanded=s4] (f3) -- (vp4) ;
\path [name path global/.expanded=s5] (f6) -- (vp5) ;

%A foreach here yields an error for some obscure reason
%\foreach \i [count=\j from 2] in {1,...,5}{
%\draw [name intersections={of=r\i and s\i}, very thick] (vp\i) -- (intersection-1) node[vertex] (ref\j) {} ;
%}
\draw [name intersections={of=r1 and s1}, very thick] (vp1) -- (intersection-1) node[vertex] (ref2) {} ;
\draw [name intersections={of=r2 and s2}, very thick] (vp2) -- (intersection-1) node[vertex] (ref3) {} ;
\draw [name intersections={of=r3 and s3}, very thick] (vp3) -- (intersection-1) node[vertex] (ref4) {} ;
\draw [name intersections={of=r4 and s4}, very thick] (vp4) -- (intersection-1) node[vertex] (ref5) {} ;
\draw [name intersections={of=r5 and s5}, very thick] (vp5) -- (intersection-1) node[vertex] (ref6) {} ;

\foreach \i in {2,...,6}{
\draw[very thick] (ref\i) -- (vp\i) ;
}

\path [name path=r6] (f1) -- (vp6) ;
\draw [name intersections={of=r6 and s5}, very thick] (vp6) -- (intersection-1) node[vertex] (ref7) {} ;
\draw[very thick] (ref7) -- (q3) ;

\path [name path=r0] (p4) -- (vp6) ;
\path [name path=s0] (e4) -- (vp1) ;
\draw [name intersections={of=r0 and s0}, very thick] (vp1) -- (intersection-1) node[vertex,label=above:$h$] (ref1) {} ;

\path [name path=y1] (v1) -- ($(p4)!-2cm!(v1)$);
\path [name path=y2] (v6) -- ($(ref1)!-2cm!(v6)$);
\draw [name intersections={of=y1 and y2}, very thick] (p4) -- (intersection-1) node[vertex,label=left:$g$] (y) {} ;
\draw[very thick] (y) -- (ref1) ;
\draw[dashed, very thin] (v1) -- (p4) ;
\draw[dashed, very thin] (v6) -- (ref1) ;

\path [name path=z1] (vp1) -- ($(u2)!-2.5cm!(vp1)$);
\path [name path=z2] (vp6) -- ($(u1)!-2cm!(vp6)$);
\draw [name intersections={of=z1 and z2}, very thick] (u1) -- (intersection-1) node[vertex,label=left:$b$] (z) {} ;
\draw[very thick] (z) -- (u2) ;
\draw[dashed, very thin] (vp1) -- (u2) ;
\draw[dashed, very thin] (vp6) -- (u1) ;

\foreach \i in {1,...,4}{
\node[inner sep=0.2cm] (ep\i) at (e\i) {} ;
\node (wp\i) at (ep\i.west) {$p_\i$};
}

\foreach \i in {3,...,6}{
\node[inner sep=0.2cm] (fp\i) at (f\i) {} ;
\node (xp\i) at (fp\i.east) {$q_\i$};
}
\end{tikzpicture}
}
\caption{Vertex linker gadget. We omitted the superscript $j$ in all the labels. Here, $\sigma_j(1)=4,~\sigma_j(2)=2,~\sigma_j(3)=5,~\sigma_j(4)=3,~\sigma_j(5)=6,~\sigma_j(6)=1$.}
\label{fig:linker-vg}
\end{figure}

The following lemma formalizes how exactly vertex $\alpha^j_i$ and vertex $\beta^j_i$ are linked: say, one chooses to put a guard on vertex $\alpha^j_i$, then the only way to see fully $\mathcal P_j$ by putting a guard at a vertex among $\beta^j_1, \ldots, \beta^j_t$ is to place it at vertex $\beta^j_i$.

\begin{lemma}\label{lem:linker-vg}
For any $j \in [k]$, the sub-polygon $\mathcal P_j$ is seen entirely by $\{\alpha^j_v, \beta^j_w\}$ iff $v = w$.
\end{lemma}

% \appendixproof{Lemma~\ref{lem:linker-vg}}
% {
\begin{proof}
The regions of $\mathcal P_j$ not seen by $\alpha^j_v$, i.e., $\mathcal P_j \setminus V(\alpha^j_v)$ consist of triangle $d^jr^j_{\downarrow}p^j_v$, triangle $x^jr^j_{\uparrow}q^j_v$ and a part of triangle $a^jb^jc^j$.
Triangle $a^jb^jc^j$ is anyway entirely seen by vertex $\beta^j_i$, for any $i \in [t]$.
It remains to prove that $d^jr^j_{\downarrow}p^j_v \cup x^jr^j_{\uparrow}q^j_v  \subseteq V(\beta^j_w)$ iff $v=w$.

It holds that $d^jr^j_{\downarrow}p^j_v \cup x^jr^j_{\uparrow}q^j_v  \subseteq V(\beta^j_v)$ since, by construction, the two reflex vertices neighboring $\beta^j_v$ are such that $\beta^j_v$ sees $\seg(d^j,p^j_\alpha)$ (hence, the whole triangle $d^jr^j_{\downarrow}p^j_v$) and $\seg(x^j,q^j_\alpha)$ (hence, the whole triangle $x^jr^j_{\uparrow}q^j_v$).   
Now, let us assume that $v \neq w$.
If $v < w$, the interior of the segment $\seg(p_v,p_w)$ is not seen by $\{\alpha^j_v, \beta^j_w\}$, and if $v > w$, the interior of the segment $\seg(q_v,q_w)$ is not seen by $\{\alpha^j_v, \beta^j_w\}$.
\end{proof}
% }

The issue we now have is that one could decide to place a guard on a vertex $\alpha^j_i$ another guard on one reflex vertex between $\beta^j_{\sigma_j(w)}$ and $\beta^j_{\sigma_j(w+1)}$ (for some $w \in [t-1]$).
This is indeed another way to guard the whole $\mathcal P_j$.
We now describe a sub-polygon $\mathcal F_j$ (for each $j \in [k]$) called \emph{linker gadget} (see Figure~\ref{fig:filter-vg}) where all the triangular pockets of $\mathcal F_j$ can be guarded by adding only one guard at a vertex of $\mathcal F_j$ iff a vertex $\beta^j_i$ has been taken in $\mathcal P_j$.
It is again based on Lemma~\ref{lem:linking-set-system:pg&vg}.

Let $d^j_1, \ldots, d^j_t$ be $t$ consecutive vertices of a regular, say, $20t$-gon, so that the angle made by $\ray(d^j_1,d^j_2)$ and the $x$-axis is a bit below $45^\circ$, while the angle made by $\ray(d^j_{t-1},d^j_t)$ and the $x$-axis is a bit above $45^\circ$. 
The vertices $d^j_1, \ldots, d^j_t$ can therefore be seen as the discretization of an arc $\mathcal C$.
We now mentally draw two lines $\ell_h$ and $\ell_v$; $\ell_h$ is a horizontal line a bit below $d^j_1$, while $\ell_v$ is a vertical line a bit to the right of $d^j_t$.
We put, for each $i \in [t]$, a vertex $x^j_i$ at the intersection of $\ell_h$ and the tangent to $\mathcal C$ passing through $d^j_i$.
Then, for each $i \in [t-1]$, we set a triangular pocket $\mathcal P(x^j_i)$ rooted at $x^j_i$ and supported by $\ray(x^j_i,d^j_1)$ and $\ray(x^j_i,\beta^j_{\sigma_j(i+1)})$.
Remark that, for convenience, on Figure~\ref{fig:filter-vg}, each point $\beta^j_{\sigma_j(i)}$ is also denoted by $c^j_i$.
%\footnote{$\beta^j_{\sigma_j(i+1)}$ is also denoted by $c^j_{i+1}$ on Figure~\ref{fig:filter-vg}.}.
We also set a triangular pocket $\mathcal P(x^j_t)$ rooted at $x^j_t$ and supported by $\ray(x^j_t,d^j_1)$ and $\ray(x^j_t,d^j_t)$.
Similarly, we place, for each $i \in [t-1]$, a vertex $y^j_i$ at the intersection of $\ell_v$ and the tangent to $\mathcal C$ passing through $d^j_{i+1}$. 
Finally, we set a triangular pocket $\mathcal P(y^j_i)$ rooted at $y^j_i$ and supported by $\ray(y^j_i,\beta^j_{\sigma_j(i)})$ and $\ray(y^j_i,d^j_t)$, for each $i \in [t-1]$ (see Figure~\ref{fig:filter-vg}).
We denote by $\mathcal P(\mathcal F_j)$ the $2t-1$ triangular pockets of $\mathcal F_j$.

\begin{figure}[h]
\centering
\resizebox{250pt}{!}
{
\begin{tikzpicture}[scale=0.68]
\node[vertex,label=right:$d_1$] (a1) at (0,0) {} ;
\path (a1)--++(65:1) node[vertex,label=right:$d_2$] (a2) {} ;
\path (a2)--++(55:1) node[vertex,label=right:$d_3$] (a3) {} ;
\path (a2)--++(60:0.5) coordinate (aa2) {} ;

\path (a3)--++(45:1) node[vertex,label=below:$d_4$] (a4) {} ;
\path (a3)--++(50:0.5) coordinate (aa3) {} ;

\path (a4)--++(35:1) node[vertex,label=below:$d_5$] (a5) {} ;
\path (a4)--++(40:0.5) coordinate (aa4) {} ;

\path (a5)--++(25:1) node[vertex,label=below:$d_6$] (a6) {} ;
\path (a5)--++(30:0.5) coordinate (aa5) {} ;

\path (a6)--++(20:0.5) coordinate (aa6) {} ;

\draw[very thick] (a1) -- (a2) -- (a3) -- (a4) -- (a5) -- (a6) ;

\node[vertex,label=below:$x_1$] (x1) at (0,-1) {} ;
\draw[very thick] (a1) -- (x1) ;
\path [name path = c] (0,-1) -- (-9,-1) ;
\path [name path= d1] (a2) -- ($(aa2)!3cm!(a2)$);
\path [name path= d2] (a3) -- ($(aa3)!5cm!(a3)$);
\path [name path= d3] (a4) -- ($(aa4)!7cm!(a4)$);
\path [name path= d4] (a5) -- ($(aa5)!10cm!(a5)$);
\path [name path= d5] (a6) -- ($(aa6)!15cm!(a6)$);

\foreach \i [count=\j from 2] in {1,...,5}{
\draw [name intersections={of=c and d\i}, dotted] (a\j) -- (intersection-1) node[vertex,label=below:$x_\j$] (x\j) {} ;
}

\begin{scope}[opacity=0.3,yshift=1cm, xshift=-2cm, rotate=0]
\foreach \i in {1,...,6}{
\node[vertex,label=above:$c_\i$] (b\i) at (-7+\i,9) {};
}
\node[vertex] (zr1) at (-5.4,8.94) {} ;
\node[vertex] (zr2) at (-4.5,8.94) {} ;
\node[vertex] (zr3) at (-3.6,8.94) {} ;
\node[vertex] (zr4) at (-2.4,8.94) {} ;
\node[vertex] (zr5) at (-1.5,8.94) {} ;


\foreach \i [count=\j from 2] in {1,...,5}{
\draw[very thick] (b\i) -- (zr\i) ;
\draw[very thick] (zr\i) -- (b\j) ;
}
\end{scope}

\path [name path = g] (0,-0.8) -- (-9,-0.8) ;

\foreach \i [count=\j from 2] in {1,...,5}{
\draw[name path global/.expanded=f\i,very thin] (x\i) -- (b\j) ;
}
\path [name path = f6] (x6) -- (a6) ;

\foreach \i in {2,...,6}{
\draw [name path global/.expanded= h\i, very thin] (x\i) -- (a1) ;
}

\foreach \i in {2,...,6}{
\draw [name intersections={of=g and h\i}, very thick] (x\i) -- (intersection-1) coordinate (z\i) {} ;
}

\foreach \i in {1,...,6}{
\draw [name intersections={of=g and f\i}, very thick] (x\i) -- (intersection-1) coordinate (w\i) {} ;
}

\foreach \i [count=\j from 2] in {1,...,5}{
\draw[very thick] (w\i) -- (z\j) ;
}

\path [name path = l] (4.5,3.4) -- (4.5,9) ;
\path [name path= m2] (a2) -- ($(aa2)!-8cm!(a2)$);
\path [name path= m3] (a3) -- ($(aa3)!-6cm!(a3)$);
\path [name path= m4] (a4) -- ($(aa4)!-4cm!(a4)$);
\path [name path= m5] (a5) -- ($(aa5)!-2cm!(a5)$);
\draw [name intersections={of=l and m2}, dotted] (a2) -- (intersection-1) node[vertex,label=right:$y_1$] (y1) {} ;
\draw [name intersections={of=l and m3}, dotted] (a3) -- (intersection-1) node[vertex,label=right:$y_2$] (y2) {} ;
\draw [name intersections={of=l and m4}, dotted] (a4) -- (intersection-1) node[vertex,label=right:$y_3$] (y3) {} ;
\draw [name path= k5,name intersections={of=l and m5}, dotted] (a5) -- (intersection-1) node[vertex,label=right:$y_4$] (y4) {} ;

\node[vertex,label=right:$y_5$] (y5) at (4.5,3.4) {};
\draw[very thick] (y5) -- (a6) ;

\path [name path = p] (4.3,3.4) -- (4.3,10) ;
\foreach \i [count=\j from 2] in {1,...,5}{
\draw [name path global/.expanded= j\j, very thin] (y\i) -- (b\i);
\draw [name intersections={of=p and j\j}, very thick] (y\i) -- (intersection-1) coordinate (za\j) {} ;
}

\foreach \i [count=\j from 2] in {1,...,4}{
\draw[name path global/.expanded= k\j,very thin] (y\i) -- (a6) ;
\draw [name intersections={of=p and k\j}, very thick] (y\i) -- (intersection-1) coordinate (zb\j) {} ;
}

\foreach \i [count=\j from 3] in {2,...,5}{
\draw[very thick] (za\j) -- (zb\i) ;
}
\end{tikzpicture}
}
\caption{The filter gadget $\mathcal F_j$. Again, we omit the superscript $j$ on the labels. Vertices $c_1, c_2, \ldots, c_t$ are not part of $\mathcal F_j$ and are in fact the vertices $\beta^j_{\sigma_j(1)}, \beta^j_{\sigma_j(2)}, \ldots, \beta^j_{\sigma_j(t)}$ and the vertices in between the $c_i$'s are the reflex vertices that we have to \emph{filter out}.}
\label{fig:filter-vg}
\end{figure}

\begin{lemma}\label{lem:filter-vg}
For each $j \in [k]$, the only ways to see entirely $\mathcal P(\mathcal F_j)$ and triangle $a^jb^jc^j$ with only two vertices of $\mathcal P_j \cup \mathcal F_j$ is to choose vertices $c^j_i$ and $d^j_i$ $($for any $i \in [t]$$)$.
\end{lemma}

% \appendixproof{Lemma~\ref{lem:filter-vg}}
% {
\begin{proof}
Proving this lemma will, in particular, entail that it is not possible to see entirely $\mathcal P(\mathcal F_j)$ with only two vertices if one of them is a reflex vertex between $c^j_i$ and $c^j_{i+1}$.
Let us call such a vertex an intermediate reflex vertex (in color class $j$).
Because of pocket $a^jb^jc^j$, one should put a guard on a $c^j_i$ (for some $i \in [t]$) or on an intermediate reflex vertex in class $j$.
As vertices $a^j$, $b^j$, and $c^j$ do not see anything of $\mathcal P(\mathcal F_j)$, placing the first guard at one of those three vertices cannot work as a consequence of what follows.

Say, the first guard is placed at $c^j_i$ ($=\beta^j_{\sigma(i)}$). 
The pockets $\mathcal P(x^j_1), \mathcal P(x^j_2), \ldots, \mathcal P(x^j_{i-1})$ and $\mathcal P(y^j_i), \mathcal P(y^j_{i+1}), \ldots, \mathcal P(x^j_{t-1})$ are entirely seen, while vertices $x^j_i, x^j_{i+1}, \ldots, x^j_t$ and $y^j_1, y^j_2, \ldots,$ $y^j_{i-1}$ are not.
The only vertex that sees simultaneously all those vertices is $d^j_i$.
It turns out that $d^j_i$ \emph{even} sees the whole pockets $\mathcal P(x^j_i), \mathcal P(x^j_{i+1}), \ldots, \mathcal P(x^j_t)$ and $\mathcal P(y^j_1), \mathcal P(y^j_2), \ldots, \mathcal P(y^j_{i-1})$.
Therefore, all the pockets $\mathcal P(\mathcal F_j)$ are fully seen.

Now, say, the first guard is put at an intermediate reflex vertex $r$ between $c^j_i$ and $c^j_{i+1}$ (for some $i \in [t-1]$).
Both vertices $x^j_i$ and $y^j_i$, as well as $x^j_t$, are not seen by $r$ and should therefore be seen by the second guard.
However, no vertex simultaneously sees those three vertices.  
\end{proof}
% }

The permutation $\sigma$ is encoded the following way. 
We position the vertex linkers $\mathcal P_1, \mathcal P_2,$ $\ldots, \mathcal P_k$ such that $\mathcal P_{i+1}$ is below and slightly to the left of $\mathcal P_i$. 
Far below and to the right of the $\mathcal P_i$'s, we place the $\mathcal F_i$'s such that the uppermost vertex of $\mathcal F_{\sigma(i)}$ is close and connected to the leftmost vertex of $\mathcal F_{\sigma{i+1}}$, for all $i \in [t-1]$.
We add a constant number of vertices in the vicinity of each $\mathcal P_j$, so that the only filter gadget that vertices $\beta^j_1, \ldots, \beta^j_t$ can see is $\mathcal F_{\sigma(j)}$ (see Figure~\ref{fig:overall-vg}).
As for the point guard version, we place in a vertical wall (\emph{Track $1$}) far from the $\alpha^j_i$'s, one triangular pocket $\mathcal P(z_{A,q})$ rooted at vertex $z_{A,q}$ and supported by $\ray(z_{A,q},\alpha^j_i)$ and $\ray(z_{A,q},\alpha^{j'}_{i'})$, for each $A$-interval $I_q=[a^j_i,a^{j'}_{i'}] \in \mathcal S_A$.
Finally, we place in a vertical wall (\emph{Track $2$}) far from the $d^j_i$'s, one triangular pocket $\mathcal P(z_{B,q})$ rooted at vertex $z_{B,q}$ and supported by $\ray(z_{B,q},d^j_i)$ and $\ray(z_{B,q},d^{j'}_{i'})$, for each $B$-interval $I_q=[b^j_{\sigma_j(i)},b^{j'}_{\sigma_{j'}(i')}] \in \mathcal S_B$.
This ends the construction (see Figure~\ref{fig:overall-vg}).

\begin{figure}[h]
\centering
\resizebox{200pt}{!}
{
\includegraphics{VertexGuardBigPictureSmall}
}
\caption{Overall picture of the reduction with $k=5$.}
\label{fig:overall-vg}
\end{figure}

We now prove the correctness of the reduction.
Assume that $\mathcal I$ is a YES-instance and let $\{(a^1_{s_1},b^1_{s_1}), \ldots, (a^k_{s_k},b^k_{s_k})\}$ be a solution.
We claim that the set of vertices $G=\{\alpha^1_{s_1}, \beta^1_{s_1}, d^1_{\sigma^{-1}_1(s_1)}, \ldots, \alpha^k_{s_k}, \beta^k_{s_k}, d^k_{\sigma^{-1}_k(s_k)}\}$ guard the whole polygon $\mathcal P$.
By Lemma~\ref{lem:linker-vg}, for each $j \in [k]$, the sub-polygon $\mathcal P_j$ is entirely seen, since there are guards on $\alpha^j_{s_j}$ and $\beta^j_{s_j}$.
By Lemma~\ref{lem:filter-vg}, for each $j \in [k]$, all the pockets of $\mathcal P(\mathcal F_j)$ are entirely seen, since there are guards on $\beta^j_{s_j}=c^j_{\sigma^{-1}_j(s_j)}$ and $d^j_{\sigma^{-1}_j(s_j)}$.
For each $A$-interval (resp.~$B$-interval) in $\mathcal S_A$ (resp.~$\mathcal S_B$) there is at least one $2$-element $(a^j_{s_j},b^j_{s_j})$ such that $a^j_{s_j} \in \mathcal S_A$ (resp. $b^j_{s_j} \in \mathcal S_B$).
Thus, the corresponding pocket is guarded by $\alpha^j_{s_j}$ (resp.~$d^j_{\sigma^{-1}_j(s_j)}$).
The rest of the polygon is seen by, for instance, $d^{\sigma(1)}_{\sigma^{-1}_{\sigma(1)}(s_{\sigma(1)})}$ and $d^{\sigma(k)}_{\sigma^{-1}_{\sigma(k)}(s_{\sigma(k)})}$.

Assume now that there is no solution to the instance $\mathcal I$ of \shs, and, for the sake of contradiction, that there is a set $G$ of $3k$ vertices guarding $\mathcal P$.
For each $j \in [k]$, vertices $b^j$, $g^j$, and $x^j_t$ are seen by three disjoint set of vertices.
The first two sets are contained in the vertices of sub-polygon $\mathcal P_j$ and the third one is contained in the vertices of $\mathcal F_j$.
Therefore, to see entirely $\mathcal P_j \cup \mathcal P(\mathcal F_j)$, three vertices are necessary.
Over all the $k$ color classes, this corresponds already to $3k$ vertices which is the size of the supposed $G$.
Thus, there should \emph{exactly} $3$ guards placed among the vertices of $\mathcal P_j \cup \mathcal F_j$.
Therefore, by Lemma~\ref{lem:filter-vg}, there should be an $s_j \in [t]$ such that both $d^j_{s_j}$ and $c^j_{s_j}=\beta^j_{\sigma_j(s_j)}$ are in $G$.
Then, by Lemma~\ref{lem:linker-vg}, a guard should be placed at vertex $\alpha^j_{\sigma_j(s_j)}$.
Indeed, the only vertices seeing $g^j$ are $f^j, g^j, h^j$ and $a^j_1, \ldots, a^j_t$; but, if the third guard is placed at vertex $f^j$, $g^j$, or $h^j$, then vertices $\beta^j_w$ (with $w \neq \sigma_j(i)$) are not seen.
So far, we showed that $G$ should be of the form $\{\alpha^1_{\sigma_1(s_1)}, \beta^1_{\sigma_1(s_1)}, d^1_{s_1}, \ldots, \alpha^j_{\sigma_j(s_j)}, \beta^j_{\sigma_j(s_j)}, d^j_{s_j}, \ldots, \alpha^k_{\sigma_k(s_k)}, \beta^k_{\sigma_k(s_k)}, d^k_{s_k},\}$.
Though, as there is no solution to $\mathcal I$, there should be a set in $\mathcal S_A \cup \mathcal S_B$ that is not hit by $\{(a^1_{\sigma_1(s_1)},b^1_{\sigma_1(s_1)}), \ldots, (a^k_{\sigma_k(s_k)},b^k_{\sigma_k(s_k)})\}$.
By construction, the pocket associated to this set is not entirely seen.

Let us bound the number of vertices of $\mathcal P$.
Each sub-polygon $\mathcal P_j$ or $\mathcal F_j$ contains $O(t)$ vertices. 
\emph{Track $1$} contains $3|\mathcal S_A|$ vertices and \emph{Track $2$} contains $3|\mathcal S_B|$ vertices. 
Linking everything together requires $O(k)$ additional vertices.
So, in total, there are $O(kt+|\mathcal S_A|+|\mathcal S_B|)$ vertices.
Thus, this reduction together with Corollary~\ref{cor:main} implies that \vgag is $\wone$-hard and cannot be solved in time $n^{o(k / \log k)}$, where $n$ is the number of vertices of the polygon and $k$ the number of guards, unless the ETH fails.
\end{proof}


